Conflict-Free Coloring: Graphs of Bounded Clique Width and Intersection Graphs

A conflict-free coloring of a graph $G$ is a (partial) coloring of its vertices such that every vertex $u$ has a neighbor whose assigned color is unique in the neighborhood of $u$. There are two variants of this coloring, one defined using the open neighborhood and one using the closed neighborhood. For both variants, we study the problem of deciding whether the conflict-free coloring of a given graph $G$ is at most a given number $k$. In this work, we investigate the relation of clique-width and minimum number of colors needed (for both variants) and show that these parameters do not bound one another. Moreover, we consider specific graph classes, particularly graphs of bounded clique-width and types of intersection graphs, such as distance hereditary graphs, interval graphs and unit square and disk graphs. We also consider Kneser graphs and split graphs. We give (often tight) upper and lower bounds and determine the complexity of the decision problem on these graph classes, which improve some of the results from the literature. Particularly, we settle the number of colors needed for an interval graph to be conflict-free colored under the open neighborhood model, which was posed as an open problem.

==> Unused/block_charac.tex <==
\section{ Proof of Lemma \ref{lem:blockon2}}\label{app:block_charac}


We give a constructive algorithm that given a block graph $G$ outputs a \cfon{}-coloring $C$ using at most three colors $1,2,3$.
For convenience, let us also specify a mapping $h$ that maps each vertex $v \in G$ to one of its uniquely colored neighbors $w \in N(v)$.
We use the fact that block-graphs are exactly the diamond-free chordal graphs (a diamond is a $K_4$ with one edge removed) 
%\tikz \draw (0pt,0pt) -- (8pt,6pt) -- (18pt, 6pt) -- (10pt,0pt) -- (0pt,0pt) (8pt,6pt)--(10pt,0pt); 
\cite{DistHere_Bandelt}.
As usual, we assume that $G$ is connected and contains at least one edge $uv$.
Color $C(u)=1$ and $C(v)=2$.
%and have $h(u)=v$ and $h(v)=u$. 
%\bscomment{May be we don't require to give h(u) and h(v). The exclusion of \{u\} and N[v] from the last sentence, works for u and v also}
Color every vertex $w \in (N(u) \cup N(v)) \setminus \{u, v\} $ with $C(w)=3$.
Assign $h(w)=v$ for every $w \in N(v)$, and assign $h(w)=u$ for every $w \in N(u) \setminus N(v)$.
%Assign $h(w)=v$ for every $w \in N(v) \setminus \{u\}$, and assign $h(w)=u$ for every $w \in N(u) \setminus N[v]$.

Let $G_v$ contain every connected component of $G \setminus \{u,v\}$ that contains a vertex from $N(v)$.
Similarly, let $G_u$ contain every connected component of $G \setminus \{u,v\}$ that contains a vertex from $N(u) \setminus N(v)$.

\begin{claim}
The sets $V(G_u)$ and $V(G_v)$ are disjoint.
\end{claim}

\begin{proof}
We first claim that $N(v) \setminus \{u\}$ and $N(u) \setminus N[v]$ are non-adjacent.
Assume, for the sake of contradiction, that there are adjacent vertices $y \in N(v) \setminus \{u\}$ and $z \in N(u) \setminus N[v]$.
Note that $v$ and $z$ are non-adjacent by definition.
Thus if also $u$ and $y$ are non-adjacent, then $uvyz$ induces a cycle of lenth four,
    in contradiction that $G$ is chordal.
Hence $uy \in E(G)$, but then $uvyz$ induces a diamond subgraph,
    in contradiction that $G$ is diamond-free.
Therefore $N(v) \setminus \{u\}$ and $N(u) \setminus N[v]$ are non-adjacent.

We now proceed to show that $V(G_u)$ and $V(G_v)$ are disjoint.
Assume, for the sake of contradiction, that $V(G_u)$ and $V(G_v)$ are not disjoint.
Since $N(v) \setminus \{u\}$ and $N(u) \setminus N[v]$ are non-adjacent, graph $G - \{u,v\}$ contains a vertex $x \in V(G) \setminus (N(u) \cup N(v))$ that is connected to $N(u)$ and $N(v)$. %\bscomment{a vertex in $G_u$ and $G_v$ ?}
We may assume that $x$ is adjacent to a vertex $y \in N(v)$ and is connected to some vertex $z \in N(u) \setminus N[v]$ by some shortest path $P_z$ in graph $G - \{u,v\}$.
Then $P_z$ together with edge $yx$ is a path of length at least two,
    which does not contain any chord since it is a shortest path.
Further, $yvuz$ or $yuz$ is a shortest path between $y$ and $z$ in graph $G[N(u) \cup N(v)]$, depending on whether $uy \in E(G)$.
Let $P'$ be this path, which has length at least two.
Then $P'$ together with $P_z$ and the edge $xy$ is a cycle of length at least four.
It has no chords since $u$ and $v$ are not adjacent to vertices of $P_z$ beside $z$.
%Thus $P'$ together with $P_z$  induces a cycle of length at least four,
This contradicts the fact that $G$ is chordal. 
\qed
\end{proof}

We color every vertex $x \in V(G_v)$ in distance $2,3,4,5,6,7,\dots$ from $v$ in graph $G_v$ with colors $1,2,3,1,2,3, \dots$  periodically.
We assign $h(x)$ for $x \in V(G_v)$ in distance $i \geq 2$ to $v$ to an arbitrary neighbor $y \in N(x)$ that has distance $i-1$ to $v$ in graph $G_v$. 
Similarly we color every vertex $x \in V(G_u)$ in distance $2,3,4,5,6,7,\dots$ from $u$ in $G_u$
with colors $2,1,3,2,1,3, \dots$  periodically.
Again, let $h(x)$ for $x \in V(G_u)$ in distance $i \geq 2$ to $u$ map to an arbitrary neighbor $y \in N(x)$ in distance $i-1$ to $u$ in graph $G_u$.

\medskip

For correctness it remains to show that $C(h(x))$ for every vertex $x \in V(G)$ occurs only once in $N(x)$.

Consider a vertex $w \in N(v)$.
Then $h(w)=v$ of color $2$.
Every other neighbor of $w$ has color $1$ or $3$, and hence $h(w)$ is a uniquely colored neighbor.

Consider a vertex $w \in N(u) \setminus N(v)$.
Then $h(w)=u$ of color $1$.
Every other neighbor of $w$ has color $2$ or $3$, and hence $h(w)$ is a uniquely colored neighbor.

Consider a vertex $w \in V(G_v)$ with some distance $i\geq 2$ to $v$.
Then $h(w)$ has distance $i-1$ to $v$.
Neighbors of $w$ may only have distance $i-1$, $i$ or $i+1$ to $v$,
    and the neighbors at different distances to $v$ have distinct colors.
Thus to prove that $h(w)$ is a uniquely colored neighbor of $w$, we have to show that there is no $w' \in N(w) \setminus \{h(w)\}$ in distance $i-1$ to $v$.
Assume, for the sake of contradiction, that there is a neighbor $w' \in N(w) \setminus \{h(w)\}$.
If $w'$ and $h(w)$ have a common neighbor $w''$ in distance $i-2$ to $v$,
    then $w''w \notin E(G)$ such that $w,h(w),w',w''$ induce a diamond subgraph or a cycle of length four,
     in contradiction to that $G$ is chordal and diamond-free.
Else, $w'$ and $h(w)$ are connected to some $w''$ with maximal distance $j< i-2$ to $v$,
    possibly $v$ itself.
Let $P_v$ be the shortest path between $w'$ and $h(w)$ going through $w''$ and using vertices with distance $\leq i-2$ to $v$.
Then $P_v$ has distance at least three and contains no chord.
Further, either $h(w)w'$ or $h(w)ww'$ is a path with no chord, which we denote as $P'$ and which has length at least one.
Then $P_v$ together with $P'$ induces a cycle of length at least four,
    in contradiction to that $G$ is chordal. 



==> Unused/blockgraphs.tex <==
\section{Block Graphs and Cographs}\label{sec:block}

In this section, we study the problems on block graphs and cographs. Note that
block graphs have clique width at most 3, and cographs have clique width at most 2. Hence, \cfonp{} and \cfcnp{} problems are polynomial time solvable on block graphs and cographs by Theorems \ref{thm:cwonp} and \ref{thm:cwcn} respectively. However, we present direct proofs for these problems on these graph classes.
In particular we show that $\chionp{}\leq 3$ and $\chicnp{}\leq 2$, for block graphs $G$. 
We show a block graph $G$ such that $\chionp{}=3$, making the above bound tight. 
Next, we show that $\chionp{}, \chicnp{}\leq 2$, for cographs $G$.

%cographs can be colored by at most 2 colors, for both problems \cfonp{} and \cfcnp{}.

%In this section, we study the problems on block graphs and cographs. Note that
%block graphs have clique width at most 3, and cographs are exactly the set of
%graphs of clique width 2. 
%\subsection{Block Graphs}

%We first consider the problem on block graphs. We show that
%$\chionp{}\leq 3$ 
%and $\chicnp{}\leq 2$, for block graphs $G$. 
%We show a block graph $G$ such that $\chionp{}=3$, making the above bound tight. 
%We show that \cfcnp{} problem is polynomial time solvable on block graphs.  
%In this section, 
%we show 
%We show that 
%three colors are sufficient and sometimes necessary to \cfonp{} color an interval graph. 
%to \cfonp{} an interval graph. 
%For 
%\emph{proper interval graphs}, we show that two colors are sufficient. 
%Since block graphs have bounded clique width, 
%The \cfonp{} and \cfcnp{} problems are polynomial time solvable by Theorems \ref{thm:cwonp} and \ref{thm:cwcn} respectively. 
%However, we present a direct proof for the \cfcnp{} problem.
%a subclass of interval graphs called \emph{non-contained interval graphs}. 
%Due to space constraints, we present the proofs in 
%related to block graphs, interval graphs and split graphs in 
%Appendix \ref{app:block_charac}. 
%, \ref{app:inter_app} and \ref{app:split} respectively.







\begin{definition}[Block Graph]
A \emph{block graph} is a graph in which every 2-connected component 
is a clique. 
\end{definition}


For the {\cfonp{}} problem, we give a tight upper bound of $3$, in the following sense:
we present a graph (see Fig. \ref{figure:block:graph}) that is not \cfonp{}-colorable with colors $\{0,1,2\}$, where 0 is the dummy-color.
Complementing this result, we show that there is an algorithm that colors a given block-graph with colors $\{1,2,3\}$, thus without the need of a dummy-color $0$.


\begin{lemma}[$\star$]\label{lem:blockon2}
If $G$ is a block graph, $\chion \leq 3$,
    hence $\chionp \leq 3$.
\end{lemma}
\begin{proof}[Proof Sketch]
We give a constructive algorithm that given a block graph $G$ outputs a \cfon{}-coloring $C$ using at most three colors $1,2,3$.
For convenience, let us also specify a mapping $h$ that maps each vertex $v \in G$ to one of its uniquely colored neighbors $w \in N(v)$.
We use the fact that block-graphs are exactly the diamond-free chordal graphs (a diamond is a $K_4$ with one edge removed) 
%\tikz \draw (0pt,0pt) -- (8pt,6pt) -- (18pt, 6pt) -- (10pt,0pt) -- (0pt,0pt) (8pt,6pt)--(10pt,0pt); 
\cite{DistHere_Bandelt}.
As usual, we assume that $G$ is connected and contains at least one edge $uv$.
Color $C(u)=1$ and $C(v)=2$.
%and have $h(u)=v$ and $h(v)=u$. 
%\bscomment{May be we don't require to give h(u) and h(v). The exclusion of \{u\} and N[v] from the last sentence, works for u and v also}
Color every vertex $w \in (N(u) \cup N(v)) \setminus \{u, v\} $ with $C(w)=3$.
Assign $h(w)=v$ for every $w \in N(v)$, and assign $h(w)=u$ for every $w \in N(u) \setminus N(v)$.
%Assign $h(w)=v$ for every $w \in N(v) \setminus \{u\}$, and assign $h(w)=u$ for every $w \in N(u) \setminus N[v]$.

Let $G_v$ contain every connected component of $G \setminus \{u,v\}$ that contains a vertex from $N(v)$.
Similarly, let $G_u$ contain every connected component of $G \setminus \{u,v\}$ that contains a vertex from $N(u) \setminus N(v)$.

\begin{claim}[$\star$]
The sets $V(G_u)$ and $V(G_v)$ are disjoint.
\end{claim}


We color every vertex $x \in V(G_v)$ in distance $2,3,4,5,6,7,\dots$ from $v$ in graph $G_v$ with colors $1,2,3,1,2,3, \dots$  periodically.
We assign $h(x)$ for $x \in V(G_v)$ in distance $i \geq 2$ to $v$ to an arbitrary neighbor $y \in N(x)$ that has distance $i-1$ to $v$ in graph $G_v$. 
Similarly we color every vertex $x \in V(G_u)$ in distance $2,3,4,5,6,7,\dots$ from $u$ in $G_u$
with colors $2,1,3,2,1,3, \dots$  periodically.
Again, let $h(x)$ for $x \in V(G_u)$ in distance $i \geq 2$ to $u$ map to an arbitrary neighbor $y \in N(x)$ in distance $i-1$ to $u$ in graph $G_u$.

The full proof is provided in Appendix \ref{app:block_charac}. 
    \qed
\end{proof}




\begin{lemma}
There is block graph $G$ with $\chionp > 2$.
\end{lemma}

\begin{figure}
\vspace{-0.3cm}
\begin{center}
\begin{tikzpicture}
[scale=0.7,auto=left, node/.style={circle,fill=white, draw, scale=0.5}
	,max/.style={circle,fill=black, draw, scale=1}]

	\node[node] (m) at (0,0) {};
	\node[node] (l) at (-1,1) {};
	\node[node] (l1) at (-1,-1) {};
	\node[node] (l2) at (-3,-1) {};
	\node[node] (l3) at (-3,1) {};
	\node[node] (xl1) at (-1,-2) {};
	\node[node] (xl2) at (-4,-2) {};
	\node[node] (xl3) at (-4,2) {};

	\node[node] (r) at (1,1) {};
	\node[node] (r1) at (1,-1) {};
	\node[node] (r2) at (3,-1) {};
	\node[node] (r3) at (3,1) {};
	\node[node] (xr1) at (1,-2) {};
	\node[node] (xr2) at (4,-2) {};
	\node[node] (xr3) at (4,2) {};
	
	\node [above] at (m.north) {$m$};
	\node [above] at (l.north) {$\ell$};
	\node [right] at (l1.east) {$x^\ell_3$};
	\node [left] at (l2.west) {$x^\ell_2$};
	\node [above] at (l3.north) {$x^\ell_1$};
	\node [left] at (xl1.west) {$\overline{x}^\ell_3$};
	\node [left] at (xl2.west) {$\overline{x}^\ell_2$};
	\node [left] at (xl3.west) {$\overline{x}^\ell_1$};
	
	\node [above] at (r.north) {$r$};
	\node [left] at (r1.west) {$x^r_3$};
	\node [right] at (r2.east) {$x^r_2$};
	\node [above] at (r3.north) {$x^r_1$};
	\node [right] at (xr1.east) {$\overline{x}^r_3$};
	\node [right] at (xr2.east) {$\overline{x}^r_2$};
	\node [right] at (xr3.east) {$\overline{x}^r_1$};
	

	\foreach \s in {l,r}{
		\foreach \a in {m,\s,\s1,\s2,\s3}{
			\foreach \b in {m,\s,\s1,\s2,\s3}{
				\draw (\a) -- (\b);
			}
		}
		\foreach \a in {\s1,\s2,\s3}{
			\draw (\a) -- (x\a);
		}
	}
\end{tikzpicture}
\end{center}
\vspace{-0.3cm}
\caption{A block graph $G$ with $\chionp > 2$.}
\label{figure:block:graph}
\vspace{-0.5cm}
\end{figure}
\begin{proof}
Let $G$ have vertex set $\{\ell,m,r\} \cup \bigcup_{i \in \{1,2,3\}} \{x^\ell_i, {\overline{x}^\ell_i}, x^r_i, {\overline{x}^r_i} \}$, see also Fig. \ref{figure:block:graph}.
Let the edge set be defined by the set of maximal cliques $\{x^s_1, x^s_2, x^s_3, s, m \}$ and  $\{x^i_s, \overline{x}^i_s \}$ for every $s\in \{\ell,r\}$ and $i \in \{1,2,3\}$.
It is easy to see that $G$ is a block graph.
To prove that $\chionp > 2$, assume, for the sake of contradiction, that there is $\chionps$-coloring $C : V \to \{0,1,2\}$.
Then there is a mapping $h$ on $V$ that assigns each vertex $v \in V(G)$ its uniquely colored neighbor $w \in N(v)$.
Note that $x^s_i$, for $s\in \{\ell,r\}$ and $i \in \{1,2,3\}$, has to be colored $1$ or $2$, since it is the only neighbor of $\overline{x}^s_i$.
Further, we may assume that $h(m) \in \{\ell, x^\ell_1\}$ and $C(h(m))=2$ because of symmetry.

First consider that $h(m)=\ell$ and $C(\ell)=2$.
Then $C(x^s_i)=1$ for every $s \in \{\ell,r\}$ and $i \in \{1,2,3\}$.
It follows that $h(\ell)=m$ and hence $C(m)=2$.
Then however $\cm(N(x_1^\ell))\supseteq \ms{1,1,2,2}$, a contradiction.

Thus it remains to consider that $h(m)=x^\ell_1$ and $C(x^\ell_1)=2$.
Then $C(x^s_i)=1$ for every $x^s_i$ with $(s,i) \in \{\ell,r\} \times [3] \setminus (\ell,1)$.
It follows that $h(r)=m$ and hence $C(m)=2$.
Then however $\cm(N(\ell)) = \ms{1,1,2,2}$, also a contradiction.

Since both cases lead to a contradiction, it must be that $\chionp > 2$. 
\qed
\end{proof}


Since a block graph $G$ have clique width at most 3,
and since $\chionp{} \leq 3$, 
we may use Theorem \ref{thm:cwonp} to decide the \cfonp{} problem for block graphs in polynomial time.

\begin{corollary}
    For block graphs, \cfonp{} is polynomial time solvable. 
\end{corollary}


By observing that the number of colors required is constant,
we have the following analogous result on the \cfcnp{} problem.
    %also since we observe that the number of colors required is bounded by a constant.
%Since block graphs have 
%clique width at most 3, part of the result follows from Theorem \ref{thm:cwcn}. 
However, we also present a direct proof using a characterization of block 
graphs $G$ with $\chicnp{} = 1$. 




\begin{theorem}\label{thm:block_cfcn}
The \cfcnp{} problem is polynomial time solvable on block graphs. 
\end{theorem}



We first show that for block graph $G$, $\chicnp \leq 2$. Then we characterize block graphs which requires 1 color and otherwise. 
To show this, we use 
%Before that, we use give the definition of a 
the \emph{perfect independent dominating set}, which is 
defined as follows.  


\begin{definition}[Perfect Dominating Set]
A perfect dominating set 
is a set 
of vertices $S\subseteq V$ such that every vertex outside $S$ has exactly one neighbor in $S$. 
A perfect independent dominating set is a perfect dominating set
where $S$ is an independent set. 
\end{definition}


\begin{lemma}\label{lem:blockcn}
If $G$ is a block graph, then $\chicnp{}\leq 2$. 
\end{lemma}

\begin{proof}
Given $G$, we consider its block decomposition. The \emph{block decomposition}, denoted $T_G$,  
is a tree of the maximal 2-connected components of $G$. For details of block decomposition,
the reader is referred to \cite{Diestel}. 

We choose an arbitrary block $r\in T_G$ as the root.
Starting from $r$, we perform a level wise coloring to the blocks using the colors 1 and 2 alternately. 
For each block, we pick one vertex as the representative. We color the representative vertex alone 
and assign the remaining vertices the color 0.

For each block, the representative vertex serves as the uniquely colored neighbor.
\qed
\end{proof}





\begin{lemma}\label{lem:pidchar}
For a graph $G$, $\chicnp{} = 1$ if and only if $G$ has a perfect independent dominating set.
\end{lemma}

\begin{proof}
Suppose $G$ has a perfect independent dominating set $S$. We assign $C:V(G)\rightarrow \{1, 0\}$.
For each vertex $v \in S$, we assign $C(v) = 1$. For the rest of vertices, we assign the color 0. 
The assignment $C$ is a \cfcnp{} coloring of $G$ that uses only 1 color.

For the reverse direction, 
let $C:V(G)\rightarrow \{1,0\}$ be a \cfcnp{} coloring of $G$.
%where the color 0 indicates that the vertex is uncolored. 
Let $V_1$ be the set of vertices in $G$ that are assigned the color 1.
Since $C$ is a \cfcnp{} coloring, it follows that
%all vertices that get the color 1 should form an independent set. Which means, 
$V_1$ is an independent set and every vertex in $V \setminus V_1$ is adjacent to exactly one vertex in $V_1$. Hence, $V_1$ is a perfect independent dominating set of $G$.
\qed
\end{proof}



\begin{proof}[Proof of Theorem \ref{thm:block_cfcn}]
If $G$ is a block graph, we know that $1\leq \chicnp{}\leq 2$ by Lemma \ref{lem:blockcn}. 
We use the above characterization to check if $\chicnp{} = 1$ or $\chicnp{} = 2$. 

Given a block graph $G$, Yen and Lee \cite{per_ind_dom_block_1996} gave a 
linear time algorithm for computing a
perfect independent dominating set of $G$.
If there exists a perfect independent dominating set, the algorithm outputs the set, otherwise
the algorithm outputs that there is no such set.
Lemma \ref{lem:pidchar}, together with Yen and Lee's result gives a linear time algorithm
that tests for a given block graph $G$ whether $\chicnp{} = 1$ or $\chicnp{} = 2$. 
\qed
\end{proof}





==> Unused/cographs.tex <==
%\section{Cographs and split graphs}
%\subsection{Cographs}\label{sec:cographs}
%We now consider the problem on cographs, and obtain Theorem \ref{thm:cographs}, the proof of which is presented in Appendix \ref{app:cographs}.  

\begin{definition}[Cograph \cite{corneil1981complement}]
A graph $G$ is a \emph{cograph} if $G$ consists of a single vertex, or if it can be constructed
from a single vertex graph using the disjoint union and complement operations.
\end{definition}


\begin{theorem}\label{thm:cographs}
The \cfonp{} and the \cfcnp{} problems are polynomial time solvable on cographs. 
\end{theorem}



%\begin{theorem}\label{thm:cographs_cn}
%The \cfcnp{} problem is polynomial time solvable on cographs. 
%\end{theorem}



We show that \cfonp{} and \cfcnp{} problems are polynomial time solvable on cographs.
Recall that cographs have clique width at most 2.
We show in the following that cographs can be colored by at most 2 colors,
    for both problems \cfonp{} and \cfcnp{}.
Analogously as for the block graphs, Theorem~\ref{thm:cwonp} and Theorem~\ref{thm:cwcn} then already imply polynomial time algorithms for both problems.
Here we present characterizations of cographs that require only 1 color,
    for both problems \cfonp{} and \cfcnp{}.
This leads to more direct algoritms,
    which check if 1 color suffices by use of the characterizations.

We use the notion of modular decomposition~\cite{habib2010survey},  
%First, we define \emph{modular decomposition}, 
which was introduced by Gallai.
%~\cite{gallai1967transitiv}.
%\textcolor{red}{DO WE NEED TO CITE GALLAI?}
A set $M \subseteq V(G)$ is called a {\it module} of $G$ if all vertices of $M$ have the same set 
of neighbors in $V(G)\setminus M$.  
The \emph{trivial modules} are $V(G)$, and $\{v\}$ for all $v$.
%A \emph{prime}  graph is a graph in which all modules are trivial. 
It has been shown \cite{corneil1981complement} that the {\it modular decomposition} of a cograph $G$  is a rooted tree $M_G$ 
that has the following properties:
%\textcolor{red}{Remove definition of prime graph. Define the characterization of cographs
%in terms of its modular decomposition directly. It has been shown \cite{corneil1981complement} 
%that $G$ is a cograph if it has a modular decomposition that satisfies the following.}
\begin{enumerate}
	\setlength{\itemsep}{1pt}
	\setlength{\parskip}{0pt}
	\item The leaves of $M_G$ are the vertices of $G$.
	\item For an internal node $t$ of $M_G$, let $M(t)$ be the set of vertices of $G$ that are leaves of the subtree of 
	$M_G$ rooted at $t$. ($M(t)$ forms a module in $G$).
	\item For each internal node $t$ of $M_G$ there is a graph $G_t$ (\emph{representative graph}) with 
	$V(G_t)=\{t_1,t_2,\dots,t_r\}$, where $t_1,t_2,\dots,t_r$ are the 
	children of $t$ in $M_G$ and for  $1 \leq i<j \leq r$, $t_i$ and $t_j$ are adjacent in $G_t$ if and only if there are vertices $u \in M(t_i)$ and $v \in M(t_j)$ that are adjacent in $G$.
	\item $G_t$ is either a clique or an independent set. 
	The node $t$ is labeled \emph{series} if $G_t$ is a clique or \emph{parallel} if $G_t$ is an independent set. 
\end{enumerate}
%A graph is a cograph if and only if its modular decomposition
%tree contains only parallel and series nodes~\cite{corneil1981complement}.
The modular decomposition of a graph can be computed in linear time~\cite{cournier1994new}.
%to solve the problem on cographs. 
%\textcolor{red}{WE ARE USING 5 CITATIONS JUST FOR MODULAR GRAPHS. WE CAN REMOVE AT LEAST TWO.}



\begin{lemma}\label{lem:cographbound}
If $G=(V,E)$ is a cograph, then $\chionp{}, \chicnp{} \leq 2$. 
%\begin{enumerate}
%    \item  $1\leq \chionp{} \leq 2$.
%    \item  $1\leq \chicnp{} \leq 2$.
%\end{enumerate}
\end{lemma}

\begin{proof}
%We use the modular decomposition technique on $G$. 

%set .

Let $r$ be the root of the modular decomposition 
tree $M_G$ of $G$. 
%Let $r$ be an arbitrarily chosen root of $M_G$ 
Since $G$ is connected, $r$ is a series node. 
Let $r_1, r_2, \dots, r_\ell$ be the children of $r$.  
For each $i\in [\ell]$, we denote $G_{r_i}$ as the cograph induced by the leaves of the subtree rooted at $r_i$. 
We consider two subgraphs $G_1=G_{r_1}$ and $G_2=G\setminus G_{r_1}$. 

Now, we describe a coloring $C:V\rightarrow \{1,2,0\}$ that works as both  \cfcnp{} and \cfonp{} coloring of $G$ . 
%as follows. 
%the assignment of colors to the vertices of $G$. 
Choose two arbitrary vertices $v\in G_1$ and $v'\in G_2$ and assign $C(v)=1$ and $C(v')=2$. 
%the colors 1 and 2 respectively. 
Remaining vertices in $V\setminus \{v,v'\}$ are assigned the color 0. 
Each vertex in $G_1$ has the vertex $v'$ %as its uniquely colored neighbor. While 
and each vertex in $G_2$ has the vertex $v$ as its uniquely colored neighbor.  
%Color one vertex in $G_1$ with color 1 and one vertex in $G_2$ with the color 2. Remaining vertices are uncolored. 
%Every vertex in $G_1$ will see the color 2 as the unique color in their neighborhood. While every vertex in $G_2$ will see the color 1 as the unique color in their neighborhood. 
%This coloring works for both \cfonp{} and \cfcnp{} problems. 
\qed
\end{proof}
Now, we characterize graphs which requires one color for both the variants. 

\begin{lemma}\label{lem:cograph_cn}
Let $G=(V,E)$ be a cograph. Then $\chicnp{}=1$ if and only if $G$ contains a universal vertex.
%$\chicnp{}=1$. 
\end{lemma}
\begin{proof}
We first prove the reverse direction. 
Let $v\in V$ be a universal vertex. We assign the color 1 to $v$ and the color 0 to the remaining vertices. 
Each vertex in $G$ has the vertex $v$ as its uniquely colored neighbor. 

For the forward direction, let $C:V\rightarrow\{1,0\}$ be a \cfcnp{} coloring  of $G$. 
%that uses one color. 
Let $G_1$ and $G_2$ be the subgraphs of $G$ as defined in Lemma \ref{lem:cographbound}. 
We first show that exactly one vertex is colored 1 in $G$. 
Suppose not. Let $v,v'\in V$ be two vertices such that $C(v)=1$ and $C(v')=1$. 
If $v,v'\in V(G_1)$ (resp. $v,v'\in V(G_2))$, then none of the vertices in $G_2$ (resp. $G_1$) has a uniquely colored neighbor. 
 If $v\in V(G_1)$ and $v'\in V(G_2)$, then 
 the vertices 
 $v$ and $v'$ do not have a uniquely colored neighbor. 
%If the two colored vertices belong to $G_1$, then none of the vertices in $G_2$ has a uniquely colored neighbor. Else, if there exists a colored vertex in each of $G_1$ and $G_2$ then the colored vertices do not have a uniquely colored neighbor. 
Hence there exists exactly one vertex, say $w$, that is colored 1. 
%$v\in G$ such that $C(v)=1$. 
%WLOG let $v\in V(G_1)$ be such that $C(v)=1$. 
%the only colored vertex of $G$. 
%Since $C$ is a \cfcnp{} coloring, 
%the coloring is a \cfcnp{} coloring, 
It follows that for each vertex in $V$, the vertex $w$ is the uniquely colored neighbor. 
Hence  $w$ is a universal vertex. 
\qed
\end{proof}


\begin{lemma}\label{lem:cograph:on}
Let $G=(V,E)$ be a cograph. 
Then $\chionp{}=1$ if and only if there exists two vertices $u,v\in V$ such that $\{u,v\}\in E$, $N(u)\cup N(v)=V$ and $N(u)\cap N(v)=\emptyset$. 
    
    
    %one of the following conditions hold.  

%\begin{enumerate}
%    \item There exists two vertices $u,v\in V$ such that $\deg(u)=1$ and $\deg(v)=|V|-1$. 
%    \item There exists two vertices $u,v\in V$ such that 
%    $\{u,v\}\in E$, $N(u)\cup N(v)=V$ and $N(u)\cap N(v)=\emptyset$. 
%\end{enumerate}
\end{lemma}
\begin{proof}
%The reverse direction is easy to see. 
We first prove the reverse direction. 
Suppose $u, v\in V$ be two vertices satisfying the above conditions. 
We assign the color 1 to  the vertices 
%assign the color 1 to both 
$u, v$ and the color 0 to the vertices in $V\setminus \{u,v\}$.
For each vertex in $N(u)$, we have the vertex $u$ as its uniquely colored neighbor whereas for each vertex in $N(v)$, we have the vertex $v$ as its uniquely colored neighbor. 
%Each vertex in $V$ has its lone neighbor that is colored as it uniquely colored neighbor. 


For the forward direction, let $C:V\rightarrow\{1,0\}$ be a \cfonp{} coloring  of $G$. 
%suppose we have a \cfonp{} coloring that uses one color. 
As $C$ is a \cfonp{} coloring, there exists two vertices\footnote{In fact, the vertices $w_1$ and $w_2$ are the only vertices colored 1.} $w_1$ and $w_2$ such that $C(w_1)=C(w_2)=1$ and $\{w_1,w_2\}\in E(G)$. 
Let $G_1$ and $G_2$ be the subgraphs of $G$ as defined in Lemma \ref{lem:cographbound}. 
We first observe that either $w_1\in V(G_1)$ and $w_2\in V(G_2)$ or 
$w_2\in V(G_1)$ and $w_1\in V(G_2)$. 
Suppose not. WLOG let $w_1,w_2\in V(G_2)$. Then each vertex in $V(G_1)$ is adjacent to two vertices colored 1 and hence there is no uniquely colored neighbor for them. 
%since $G$ is connected. 
Hence WLOG, let $w_1\in V(G_1)$ and $w_2\in V(G_2)$. 


It is easy to see that $N(w_1)\cap N(w_2)=\emptyset$. Suppose not. If 
there exists a vertex $w\in N(w_1)\cap N(w_2)$, then $w$ does not have a uniquely colored neighbor. 
Also $N(w_1)\cup N(w_2)=V$. Suppose not. If there exists a vertex $w\notin N(w_1)\cup N(w_2)$,  then $w$ does not have a colored neighbor. 
%It is clear that no vertex in $V(G_2)\setminus \{w_2\}$ is adjacent to $w_2$. Else, 
%none of the vertices in $V(G_2)\setminus \{w_2\}$ has a uniquely colored neighbor. 
%Now, we comment on the vertices in $V(G_1)\setminus \{w_1\}$. 
%If there exists a vertex $w''\in V(G_1)\setminus \{w_1\}$ such that 
%$\{w'',w_2\}\in E(G)$, then $\{w'',w_1\}\notin E(G)$. So if $N(w_2)\setminus \{w_1\}=\emptyset$, we reach the condition (1), else if 
%$N(w_2)\setminus \{w_1\}\neq \emptyset$, we reach the condition (2). 
\qed
\end{proof}

Theorem \ref{thm:cographs} follows from Lemmas \ref{lem:cographbound}, \ref{lem:cograph_cn} and 
\ref{lem:cograph:on}.













Since constant bounds for the partial coloring variants imply constant bounds for the full coloring variants and since block graphs and cographs have clique width at most 3, we have the following. 
\begin{theorem}\label{thm:full_coloring_block_cographs}
The \cfon{} and the \cfcn{} problems are polynomial time solvable on block graphs and cographs. 
\end{theorem}



==> Unused/inter_app.tex <==
\section {Proof of Lemma \ref{lem:int-lb}}\label{app:inter_app}

\begin{figure}
\renewcommand\thefigure{\ref{figure:interval:lower:bound}}
%\vspace{-0.5cm}
\begin{center}
\begin{minipage}{0.4\textwidth}
\centering
%\begin{tikzpicture}[every node/.style={node distance=1.5cm,scale=0.5}, scale = 0.6]
\begin{tikzpicture}[scale = 0.6]
\tikzstyle{vertex}=[circle,draw, minimum size=3pt,node distance=1.5cm,scale=0.5]
\tikzstyle{edge} = [draw,thick,-,black]
\node[vertex]  (u1) at (1,0) {};
\node[vertex]  (u2) at (2,0) {};
\node[vertex]  (u3) at (3,0) {};
\node[vertex]  (u4) at (4,0) {};
\node[vertex]  (u5) at (5,0) {};
\node[vertex]  (u6) at (6,0) {};
\node[vertex]  (u7) at (7,0) {};
\node[vertex]  (u8) at (8,0) {};
\node[vertex]  (v1) at (2,1.5) {};
\node[vertex]  (v2) at (4.5,1.5) {};
\node[vertex]  (v3) at (7,1.5) {};
\draw[edge, color=black] (u1) -- (v1) (u2) -- (v1) (u3) -- (v1) ;
\draw[edge, color=black] (u3) -- (v2) (u4) -- (v2) (u5) -- (v2) (u6) -- (v2) ;
\draw[edge, color=black] (u6) -- (v3) (u7) -- (v3) (u8) -- (v3) ;
\draw[edge, color=black] (v1) -- (v2);
\draw[edge, color=black] (v2) -- (v3);
\node [above] at (v1.north) {$u$};
\node [below] at (u1.south) {$u'$};
\node [below] at (u2.south) {$u''$};
\node [below] at (u3.south) {$u^{\star}$};
\node [above] at (v2.north) {$v$};
\node [below] at (u4.south) {$v'$};
\node [below] at (u5.south) {$v''$};
\node [below] at (u6.south) {$w^{\star}$};
\node [below] at (u7.south) {$w'$};
\node [below] at (u8.south) {$w''$};
\node [above] at (v3.north) {$w$};
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.4\textwidth}
\centering
\begin{tikzpicture}[scale=1]
	\intervallltriple{1}{2.5}{1.9}
	
	\intervallltriple{3.5}{5}{1.9}
	
	\intervalllquadruple{1}{1.5}{1.1}
	\intervalllquadruple{1.5}{2}{1.1}
	\intervallltriple{2}{2.5}{1.3}
	\intervalllquadruple{2.5}{3}{1.3}
	\intervalllquadruple{3}{3.5}{1.3}
	\intervallltriple{3.5}{4}{1.3}
	\intervalllquadruple{4}{4.5}{1.1}
	\intervalllquadruple{4.5}{5}{1.1}

	\intervallltriple{2}{4}{0.7}
	
\end{tikzpicture}
\end{minipage}
%\vspace{-0.3cm}
\end{center}
\caption{(repeated) On the left hand side, we have the graph $G'$, and on the right hand side we have
an interval graph representation of $G$, a graph where $\chion{} > 3$.
The graph $G$ is obtained by replacing each vertex $u,v,w,u^\star,v^\star$
of $G'$ with a 3-clique and replacing each of $u',u'',v',v'',w',w''$ with a 4-clique.}
\vspace{-0.3cm}
\end{figure}
\addtocounter{figure}{-1}

We define the graph $G$,  an interval representation seen in Figure \ref{figure:interval:lower:bound}, with the help of a preliminary graph $G'=(V',E')$.
Let $V'$ consists of vertices $u,v,w$ and $u',u'',u^\star,v',v'',w^\star,\allowbreak w',\allowbreak w''$.
Let $E'$ be the edges which form the maximal cliques $\{u',u\}, \{u'',u\},\allowbreak \{u^\star,u,v\},\allowbreak \{v,v'\},\allowbreak \{v,v''\},\allowbreak \{w^\star,v,w\},\allowbreak \{w,w'\}, \{w,w''\}$.
By this ordering of maximal cliques, we observe that $G'$ is an interval graph.

The graph $G$ is obtained by replacing each vertex $u,v,w,u^\star,w^\star$
of $G'$ with a 3-clique and replacing $u',u''.v',v'',w',w''$ by a 4-clique.
Formally, that is $V(G)= \bigcup_{x \in V'} \{x_1,x_2,x_3\} \cup \{u_4',u_4''.v_4',v_4'',w_4',w_4''\}$ and $E(G) = \bigcup_{vw \in E', \; i,j \in [4]} v_i w_j$ (for those where vertices $v_i$ and $w_j$ exists).
Since $G$ is an interval graph, also $G'$ is an interval graph.

Now we show that $G$ cannot be \cfon{} colored with 3 colors.
Assume there is a \cfon{} coloring $C: V(G) \rightarrow \{1,2,3\}$.
Let $h$ map each vertex $x \in V(G)$ to a uniquely colored neighbor $y \in N(x)$.
%We use the notation $L_{uv} = \bigcup_{1\leq i \leq 3} \{u_i,v_i\}$ and 
% $L_{vw} = \bigcup_{1\leq i \leq 3} \{v_i,w_i\}$.

\begin{claim}
$|C(\{x_1,x_2,x_3\})| = 2$ for every $x \in \{u,v,w\}$.
\end{claim}
\begin{proof}[Claim's Proof]
First, let us assume, for the sake of contradiction, that $|C(\{u_1,u_2,u_3\})| = 1$, say with the coloring $C(\{u_1,u_2,u_3\})= \{1\}$.
Note that the neighborhood $N(\{u_1',u_2',u_3', u_4'\}) \subseteq \allowbreak \{u_1,u_2,u_3, u_1',u_2',u_3',u_4'\}$.
It follows for the uniquely colored neighbors $h(\{u_1',u_2',u_3', u_4'\}) \subseteq \allowbreak \{u_1',u_2',u_3', u_4'\}$,
	which then must satisfy coloring $ \{2, 3\} \subseteq C(\{u_1',u_2',u_3', u_4'\})$.
	%$\cm(\{u_1',u_2',u_3', u_4'\}) = \ms{2, 2, 3, 3}$.
Analogously it follows that $ \{2, 3\} \subseteq C(\{u_1'',u_2'',u_3'', u_4''\})$.
%$\cm(\{u_1'',u_2'',u_3'', u_4''\}) = \ms{2,2,3,3}$.
Then we have the contradiction that $C_{\{\!\!\{ \}\!\!\}}(N(u_1)) \supseteq \{\!\!\{ 1,1,2,2,3,3 \}\!\!\}$.
By symmetry the claim also follows for $x \in \{v,w\}$.

It remains to show that $|C(\{x_1,x_2,x_3\})| \neq 3$.
Assume, for the sake of contradiction, that $C(\{u_1,u_2,u_3\}) = \{1,2,3\}$.
They are adjacent to $\{v_1,v_2,v_3\}$ which as just observed have $|C(\{v_1,v_2,v_3\})| \geq 2$.
%Thus $C(L_{uv})$ has at least two colors that occur at least twice, in contradiction to the previous claim.
If $|C(\{v_1,v_2,v_3\})| = 3$, then 
%$\cm(N(u^\star_1)) \supset \ms{1,1,2,2,3,3}$
$\cm(L_{uv}) = \cm(N(u^\star_1) \setminus \{u^\star_2, u^\star_3 \}) = \ms{1,1,2,2,3,3}$, 
and $u^\star_1$ cannot have a uniquely colored neighbor.
If $|C(\{v_1,v_2,v_3\})| = 2$, then WLOG, we assume $C(v_1)=1, C(v_2)=1, C(v_3)=2$.
Then $\cm(N(u_3)) \supset \ms{1,1,2,2}$ and thus $C(h(u_3)) = 3$.
However, since $h(u_3) \in N(u_1)$, $\cm(N(u_1)) \supset \ms{1,1,2,2,3,3}$
    and $u_1$ cannot have a uniquely colored neighbor.

By symmetry, the claim also follows for $x \in \{v,w\}$.
\qed
\end{proof}

%\begin{claim}
%$C(L_{uv})$ has at most one color that occurs more than once. Symmetrically the same is true for $C(L_{vw})$.
%\end{claim}
%\begin{proof}[Claim's Proof]
%Assume, for the sake of contradiction, that there are at least two colors that occur at least twice in $C(L_{uv})$, say 1 and 2.
%
%Suppose that $3 \notin C(L_{uv})$.
%Notice that $h(u^\star_1)$ must be colored 3, and also $h(u^\star_1) \in \{u^\star_2, u^\star_3\}$.
%WLOG, let $h(u^\star_1) = u^\star_2$. This means $C(u^\star_2) = 3$ and $C(u^\star_3) \in \{1, 2\}$.
%By a similar reasoning $C(h(u^\star_2)) = 3$. This forces $h(u^\star_2) = u^\star_1$ and $C(u^\star_1) = 3$. However now
%$\cm(N(u^\star_3))= \ms{1,1,2,2,3,3}$, and leaves $u^\star_3$ without a uniquely colored neighbor. Hence $1,2,3 \in C(L_{uv})$.
%
%Note that if $\cm(L_{uv}) = \cm(N(u^\star_1) \setminus \{u^\star_2, u^\star_3 \}) = \ms{1,1,2,2,3,3}$, then $u^\star_1$ cannot have a uniquely colored neighbor. 
%Hence, 3 appears only once in $C(L_{uv})$.
%%Since 1 and 2 appear at least twice in $C(L_{uv})$, it follows that 
%%$\cm(L_{uv}) = \ms{1,1,1,2,2,3}$ or $\cm(L_{uv}) = \ms{1,1,2,2,2,3}$.
%We consider two cases.

%Now consider that either $u_1,u_2,u_3$ or $v_1,v_2,v_3$ are colored with 1,2,3, and the three vertices are colored with 1 and 2.
%%Suppose that $u_1,u_2,u_3$ is colored 1,2,3,
%%     and hence $v_1,v_2,v_3$ is colored with 1 and 2.
%By symmetry, we may assume that $C(u_1)=1,C(u_2)=2,C(u_3)=3$ and $C(v_1)=1, C(v_2)=1, C(v_3)=2$.
%Then $\cm(N(u_3)) \supset \ms{1,1,2,2}$ and thus $C(h(u_3)) = 3$.
%However, also $h(u_3) \in N(u_1)$, and hence $\cm(N(u_1)) \supset \ms{1,1,2,2,3,3}$
%    and $u_1$ cannot have a uniquely colored neighbor.
%%The analogous contradiction follows when assuming $v_1,v_2,v_3$ is colored 1,2,3,     

%In the remaining cases, up to symmetry, we can assume $C(u_1)=1,C(u_2)=1,C(u_3)\in\{1,2\}$ and $C(v_1)=2, C(v_2)=2, C(v_3)=3$.
%Then $\cm(N(v_3)) \supset \ms{1,1,2,2}$
%    and hence $C(h(v_3))=3$.
%Notice that $h(v_3) \notin \{u^\star_1, u^\star_2, u^\star_3\}$, because for instance, if
%$h(v_3) = u^\star_1$, then $\cm(N(u^\star_3)) \supseteq \ms{1,1,2,2,3,3}$.
%Thus $h(v_3) \notin \{u^\star_1, u^\star_2, u^\star_3\}$
%    and hence $h(v_3)$ is either in one of the 4-cliques replacing $v'$ or $v''$
%        or possibly one of the six vertices $w_1,w_2,w_3,w^\star_1,w^\star_2,w^\star_3$.
%Hence in both cases, there is a clique of at least four vertices $x_1,x_2,x_3,x_4 \in N(v_3) \cap N[h(v_3)]$ 
%    that are not part of $L_{uv}$.
%We may assume that $h(v_3) = x_1$.
%As mentioned above, $C(x_1) = 3$.
%Then $x \in  \{x_2,x_3,x_4\}$ has $\cm(N(x)) \supseteq \cm (\{v_1,v_2,v_3\}) \cup C(x_1) = \ms{2,2,3,3}$.
%% The following is not true.
%Therefore $x_2$ has either of $x_3,x_4$ as its uniquely colored neighbor, say $h(x_2)=x_3$, which must be of color $1$.
%Then in turn $x_3$ has either of $x_2,x_4$ as its uniquely colored neighbor, say $h(x_3)=x_2$,
%    which must also be of color $1$.
%Then, however, $x_4$ has $\cm(N(x_4)) \supseteq \ms{1,1,2,2,3,3}$
%    and therefore has no uniquely colored neighbor.
%\qed
%\end{proof}

WLOG, we may now assume that $C(v_1)=1, C(v_2) = 2, C(v_3) = 2$.
If $3 \notin C(\{u_1, u_2, u_3\})$, then $h(u^\star_1)$ must be colored 3 and be either $u^\star_2$ or $u^\star_3\}$.
WLOG, let $h(u^\star_1) = u^\star_2$. This means $C(u^\star_2) = 3$ and $C(u^\star_3) \in \{1, 2\}$.
By a similar reasoning $C(h(u^\star_2)) = 3$. This forces $h(u^\star_2) = u^\star_1$ and $C(u^\star_1) = 3$. However now
$\cm(N(u^\star_3)) \supset \ms{1,1,2,2,3,3}$, and leaves $u^\star_3$ without a uniquely colored neighbor. Hence, $3 \in C(\{u_1, u_2, u_3\})$, analogously, $3 \in C(\{u_1, u_2, u_3\})$.

However, $v_1$ is now adjacent to at least two vertices of color 3 and two of color 2.
Hence, $v_1$ must be adjacent to exactly one vertex with color 1.
This implies either $1 \notin C(\{u_1, u_2, u_3\})$ or $1 \notin C(\{w_1, w_2, w_3\})$.
WLOG, suppose $1 \notin C(\{u_1, u_2, u_3\})$.
Hence, by the claim above, $2, 3 \in C(\{u_1, u_2, u_3\})$.

However, $v_2$ is then adjacent to two vertices with color 1 (i.e., $v_1$ and $h(v_1)$), two vertices of color 2 (i.e., one in $\{u_1, u_2, u_3\}$ and one in $\{w_1, w_2, w_3\}$), two vertices of color 3 (i.e., $v_3$ and a vertex in $\{u_1, u_2, u_3\}$).
That means it does not have a uniquely colored neighbor, a contradiction.
Therefore, $G$ cannot be \cfon{} colored with 3 colors.

%WLOG, we may now assume that $C_{\{\!\!\{ \}\!\!\}}(\{v_1,v_2,v_3\})= \{\!\!\{ 1,3,3 \}\!\!\}$
%with $C(v_1)=1$.
%The previous two claims imply that  $C_{\{\!\!\{ \}\!\!\}}(\{u_1,u_2,u_3\})= \cm ( \{w_1,w_2,w_3\}) = \{\!\!\{ 2,3,3 \}\!\!\}$.
%%as well as that $c_{\{\!\!\{ \}\!\!\}}(\{w_1,w_2,w_3\})= \{\!\!\{ 2,3,3 \}\!\!\}$.
%Now $C(h(v_1))=1$ since we already now that $C_{\{\!\!\{ \}\!\!\}}(N(v_1)) \supseteq \{\!\!\{ 2,2,3,3 \}\!\!\}$.
%Observe that $h(v_1) \in N(v_2)$. % since $N(v_1)=N(v_2)$.
%Then however $\cm(v_2) \supseteq \ms{1} \cup \ms{1,2,2,3,3}$. A contradiction.
%Thus the coloring $C$ is infeasible and $G$ cannot be $\chi_{ON}$-colored with 3 colors.


==> Unused/unit_disk_hardness.tex <==
\subsection{{\sf NP}-completeness}
In this section, we show the algorithmic result for unit disk intersection graphs and unit square intersection graphs. 
The idea of the proof is \thcomment{based (?)} on the lines with the proofs \thcomment{of ...} in \cite{Sandor_2017_interval, Boe2019}. We prove the following for the unit disk intersection graph. A similar result can be obtained for the unit square intersection graph. 
\begin{theorem}\label{thm:udick-hard}
It is {\sf NP}-complete to determine if a unit disk intersection graph $G$ can be \cfonp{} colored using one color. 
\end{theorem}
\begin{proof}
Given a unit disk intersection graph $G=(V,E)$, 
and a \cfonp{} coloring using one color, we can verify whether the coloring is a valid one. We now prove the {\sf NP}-hardness aspect of the problem. We give a reduction from the \textsc{Positive Planar 1-in-3-SAT}. 
Given a Boolean formula $\phi$, we construct a unit disk intersection graph $G(\phi)$. 
We show that 
$G(\phi)$ has a \cfonp{} coloring if an only if 
$\phi$ is 1-in-3-satisfiable. 
We now explain the construction of the graph $G(\phi)$ from $\phi$. 

\noindent
\textbf{Construction of $G(\phi)$:} Let the variables of $\phi$ be represented by $\{x_1,x_2,\dots, x_n\}$ and the clauses of $\phi$ by $\{c_1,c_2, \dots, c_k\}$. 
Each variable $x_j$ is represented by a gadget which is a  \textcolor{red}{cycle of length $8k$}. 
We start with an arbitrary vertex and designate the vertex as $a_{1j}$. The next three consecutive vertices (in anti-clockwise direction) 
are designated by $b_{1j}$, $c_{1j}$ and $d_{1j}$. 
Every fourth vertex from $a_{1j}$, $b_{1j}$, $c_{1j}$ and $d_{1j}$ are denoted as $a_{ij}$ $b_{ij}$, $c_{ij}$ and $d_{ij}$ respectively, where $i\in \{2, \dots, 2k\}$. see Figure \ref{fig:unitdisk_gadjets}. 

The clause gadget is illustrated in Figure \ref{fig:unitdisk_gadjets}. 
The thick vertex in the gadget is called the \emph{clause vertex} denoted by $c$. 
Each dotted vertex indicates the connection of the clause vertex with each of three variable gadgets that corresponds to the variables of the clause. 
We will now look at the connections between the variable gadgets and the clause gadgets. 
%The clause vertex $c$ does not have a uniquely colored neighbor from within the gadget. Hence one of its neighbors designated $d_1, d_2, d_3$ 
%will act as its uniquely colored neighbor. 
The clause vertex $c$ is connected to a variable gadget through a \textcolor{red}{path of length $4p$} \footnote{The value of $p$ differs for each connection with the variable gadget. And it is decided later. }, where $p$ is an integer.
\thcomment{I suggest to put the footnote in-text here.}
For better illustration, we show a path of length 4 in Figure \ref{fig:unitdisk_connections}. We now show that $G[\phi]$ is \cfonp{} colorable using one color  if and only if $\phi$ is 1-in-3-satisfiable. \\


%If the variable $x_j$ is set to true in $\phi$, then all the $a_{ij}$ vertices are colored and exactly one of the following holds: either all the $d_{ij}$ are colored or all the $b_{ij}$ are colored, where $i\in [2k]$. 
%Else if $x_j$ is set to false in $\phi$, then all the $c_{ij}$ are colored and exactly one of the following hold: either all $d_{ij}$ are colored or all $b_{ij}$ are colored. The remaining vertices are left uncolored in both the cases. 




\begin{figure}[t!]
\begin{center}
    
\begin{minipage}{0.4\textwidth}
\centering

\begin{tikzpicture}[every node/.style={node distance=1.8cm,scale=0.9}, scale = 0.5]

\tikzstyle{vertex}=[dot, draw, minimum size=8pt]
%\draw[gray] (-6,2.4) -- (7,2.4);
%\draw[gray] (-6,0.4) -- (7,0.4);

\draw[dotted, thick] (-4,5) circle (1cm);
\draw[dotted, thick] (-2,3) circle (1cm);
\draw[dotted, thick] (-6,3) circle (1cm);
\draw[thick] (-4,3) circle (1cm);
\draw[thin] (-4,1) circle (1cm); 
\draw[thin, shade] (-4,-1)  circle (1cm);
\draw[thin] (-6,-1)  circle (1cm);
\draw[thin, shade] (-2,-1)  circle (1cm);
\draw[thin] (0,-1)  circle (1cm);


\node at (-4,3) {$c$};
%\node at (1.2,2.6) {$v$};


\end{tikzpicture}

\end{minipage}
\begin{minipage}{0.4\textwidth}
\centering

\begin{tikzpicture}[every node/.style={node distance=1.8cm,scale=0.9}, scale = 0.5]

\tikzstyle{vertex}=[dot, draw, minimum size=8pt]
%\draw[gray] (-6,2.4) -- (7,2.4);
%\draw[gray] (-6,0.4) -- (7,0.4);

\draw[thin] (-4,5) circle (1cm);
\draw[thin] (-3,6) circle (1cm);
\draw[thin] (-4,3) circle (1cm);
\draw[thin] (-1,6) circle (1cm);


\node at (-4,5) {$c_{1j}$};
\node at (-3,6) {$b_{1j}$};

\node at (-4,3) {$d_{1j}$};
\node at (-1,6) {$a_{1j}$};

\draw[thin] (-3,-3) circle (1cm);
\draw[thin] (-1,-3) circle (1cm);
\draw[thin] (-4,-2) circle (1cm);
\draw[thin] (-4,0) circle (1cm);
%\node at (-3,-3) {$b_{21}$};
%\node at (-4,-2) {$a_{21}$};


\draw[thin] (5,-2) circle (1cm);
\draw[thin] (2,-3) circle (1cm);
\draw[thin] (4,-3) circle (1cm);
\draw[thin] (5,0) circle (1cm);


\node at (5,-2) {$c_{ij}$};
\node at (2,-3)  {$a_{ij}$};

\node at (4,-3) {$b_{ij}$};
\node at (5,0) {$d_{ij}$};

\draw[thin] (5,5) circle (1cm);
\draw[thin] (2,6) circle (1cm);
\draw[thin] (4,6) circle (1cm);
\draw[thin] (5,3) circle (1cm);

\node at (-4,1.5) {$\dots$};
\node at (0.5,-3) {$\dots$};
\node at (5,1.5) {$\dots$};
\node at (0.5,6) {$\dots$};



%\node at (1.2,2.6) {$v$};


\end{tikzpicture}
\end{minipage}
\end{center}
\caption{On the left, we have the clause gadget. The thick disk indicates the clause vertex $c$ and the dotted disks indicate the connections with the variable gadgets. 
The red \thcomment{TH: where red?} colored vertices force the clause vertex to not draw its uniquely colored neighbor from within the clause gadget. On the right we have the variable gadget for $x_j$. 
}
\label{fig:unitdisk_gadjets}


\end{figure}





\begin{figure}[t!]
\begin{center}
    
\begin{minipage}{0.4\textwidth}
\centering

\begin{tikzpicture}[every node/.style={node distance=1.8cm,scale=0.9}, scale = 0.5]

\tikzstyle{vertex}=[dot, draw, minimum size=8pt]
%\draw[gray] (-6,2.4) -- (7,2.4);
%\draw[gray] (-6,0.4) -- (7,0.4);


\draw[thin, shade] (6,1) circle (1cm);
\draw[thin, shade] (6,3) circle (1cm);
\draw[thin] (4,3) circle (1cm);
\draw[thin] (2,3) circle (1cm);
\draw[thin, shade] (0,3) circle (1cm);
\draw[thin, shade] (-2,3) circle (1cm);
\draw[thick] (-4,3) circle (1cm);
\draw[dotted, thick] (-4,1) circle (1cm); 
\draw[dotted, thick] (-4,-1)  circle (1cm);
\draw[dotted, thick] (-6,-1)  circle (1cm);
\draw[dotted, thick] (-2,-1)  circle (1cm);
\draw[dotted, thick] (0,-1)  circle (1cm);
\draw[thin] (6,5) circle (1cm);
\draw[thin] (6,-1) circle (1cm);

\node at  (6,3) {$a_{\ell j}$};
\node at  (6,1) {$b_{\ell j}$};
\node at  (6,-1) {$c_{\ell j}$};
\node at  (6,5) {$d_{\ell-1 j}$};
\node at (4,3) {$g_i$};
\node at (2,3) {$f_i$};
\node at (0,3) {$e_i$};
\node at (-2,3) {$d_i$};
\node at (-4,3) {$c$};
\node at (6,7) {$\dots$};
\node at (6,-3) {$\dots$};
%\node at (1.2,2.6) {$v$};


\end{tikzpicture}

\end{minipage}
\end{center}
\caption{Path connecting the clause vertex $c$ to the vertex $a_{\ell j}$ in variable gadget $x_j$. The dashed vertices are a part of the clause gadget. The vertices $d_i$ and $e_i$ are colored if $x_j$ is true. Else, the vertices $e_i$ and  $f_i$ are colored. Every fourth vertex from the initial colored vertices are colored along the path, starting from either $\{d_i,e_i\}$ or $\{e_i,f_i\}$. }
\label{fig:unitdisk_connections}


\end{figure}


\noindent 
\textbf{Colorability implies Satisfiabilty:} We start from the clause vertices. %Consider a clause vertex $c$. 
For each clause vertex $c$, in any \cfonp{} colorable using one color, exactly one of the vertices $d_1, d_2, d_3\in N(c)$ (which are the vertices connecting $c$ to three variables gadgets through a path)
is colored. 
This is because the shaded vertices in the clause gadget are colored and forces $c$ to not have a uniquely colored neighbor from within the gadget. 
WLOG, let $d_1$ be colored and $d_2, d_3$ be uncolored. Along the path from $d_1$ to $g_i$ which connects to a vertex $a_{ij}$ in the variable gadget, in any \cfonp{} coloring we have two colored vertices followed by two uncolored vertices and so on starting from $d_1$. 
%$a_{ij}$ be the vertex in the variable gadget connecting the path from $d_1$. 
This ensures that all the $a_{ij}$'s in $x_j$ are colored. Hence in $x_j$ either all the $d_{ij}$'s are colored or all the $b_{ij}$'s are colored and not both. 

Along the paths from $d_2$ and $d_3$ to their respective variable gadgets, we have two vertices colored and two vertices uncolored and so on starting from the neighbor of $d_2$ (other than $c$) in the path to the variable gadget. 
This ensures that $g_i$ is uncolored and has its neighbor in the path $f_i$ as its uniquely colored neighbor. 
Hence its neighbor $a_{ij}$ remains uncolored and should have its uniquely colored neighbor from within the variable gadget. 
In any \cfonp{} coloring, all the $c_{ij}$'s are colored and either all $b_{ij}$'s are colored or all $d_{ij}$'s are colored and not both. 
Note that all the $a_{ij}$'s are uncolored. 

For a \cfonp{} coloring, in a variable gadget $x_j $ if all $a_{ij}$'s are colored, we set $x_j$ to be true in $\phi$. Else we set $x_j$  to be false. 
Hence exactly one variable is set to true in each clause making it 1-in-3-satisfiable. \\ 
%Thus it forces the When $d_1$ is uncolored, it forces the vertices $g_i$ and $a_ij$ to be uncolored. Thus in any \cfonp{} coloring either $b_{ij}$ is colored or $d_{i-1}j$ is colored thereby forcing the vertices $c_{ij}$ or $c_{i-1}j$ to be colored. 
%As argued in the earlier case, because of the type of vertices colored in this coloring, this gadget implies $x_j$ should be set to false in $\phi$. 


%One of its neighbors is colored The coloring ensures that $a_{ij}$ is colored and one of $b_{ij}$ and $d_{i-1j}$ is colored. 
%If $b_{ij}$ is colored, it forces $c_{ij}$, $d_{ij}$ to be uncolored and $a_{i+1 j}$, $b_{i+1 j}$ to be colored. 
%This ensures that all $a_{ij}$ and $b_{ij}$   where $\forall 1\leq i\leq 8k$ are colored in the gadget $x_j$. 
%Else if $d_{i-1j}$ is colored, then it forces $b_{ij}$, $c_{ij}$, $b_{i-1j}$, $c_{i-1j}$ to be uncolored and $a_{ij}$, $d_{i-1 j}$ to be colored for all $i\leq 8k$. 
%Since all $a_{ij}$'s are colored and either all $b_{ij}$'s or all $d_{ij}$'s are colored, we have that $x_j$ is true in $\phi$. 


%$d_{ij}$ are uncolored and 
%viceversa. Since it is a \cfonp{} coloring, we have all the $a_{ij}$ to be colored and either all the $b_{ij}$ or all the $d_{ij}$ are colored. 




\noindent
\textbf{Satisfiability implies Colorability:}
For each variable $x_j$ that is set to true in $\phi$, we set all the $a_{ij}$'s and $b_{ij}$'s to be colored. 
Else if $x_j$ is false in $\phi$, we set all $b_{ij}$'s and $c_{ij}$'s to be colored. 
In either of the cases, the remaining vertices in the gadget are uncolored and such a coloring ensures that every vertex has a uniquely colored neighbor for every vertex in $x_j$. 
The case when all $a_{ij}$ and $b_{ij}$ are colored is illustrated in Figure \ref{fig:unitdisk_connections}. 

In the case when all $a_{ij}$'s are colored, its neighbor $g_i$ in the path (if any) is uncolored. Starting from $g_i$ to the vertex $d_i$, two vertices are uncolored and next two vertices are colored and so on. This forces the vertices $d_i, e_i$ to be colored. Else if all $a_{ij}$'s are uncolored, then its neighbor $g_i$ (if any) is uncolored and starting from $f_i$ to $d_i$, we have two vertices colored and next two vertices uncolored and so on. 
This leaves the vertex adjacent to $c$ in that path to be uncolored. 
Since $\phi$ is 1-in-3-satisfiable, exactly one of its neighbors is colored which acts as its uniquely colored neighbor. We can extend this color to each of the clause gadgets and get a \cfonp{} coloring using one color. 

%and This forces the vertex $g_i$ to be uncolored and $a_{i j}$ acts as its uniquely colored neighbor. This implies that $f_i$ is uncolored and the vertices $d_i$ and $e_i$ are colored. Now all the vertices along  the path including the clause vertex $c$ have a uniquely colored neighbor. 
%For each variable $x_j$ that is set to false in $\phi$, either all $c_{ij}$ and $d_{ij}$ are colored or 
%all 
%$c_{ij}$ and $b_{ij}$ are colored. 
%Such a coloring ensures a uniquely colored neighbor for every vertex in the gadget. Because the vertices $a_{ij}$ are uncolored and have a uniquely colored neighbor, this forces the vertex $g_i$ to be uncolored. Hence the vertices $e_i$ and $f_i$ are colored and $d_i$ is uncolored. Note that the $d_i$ connecting $c$ to a false (true) variable gadget is always uncolored (colored).  


%Since $\phi$ is 1-in-3-satisfiable, exactly one of the three vertices connecting $c$ to the variable gadgets is colored. Thus the clause variable has a uniquely colored neighbor. 

%then $d_j, e_j$ are colored and $f_j, g_j$ are uncolored. Else we have the vertices $e_i, f_i$ as colored and the vertices $d_i, g_i$ are left uncolored. 
%Note that if $x_t$ is true then $a_{j\ell}, b_{j\ell}$ are colored and $a_{j\ell}$ serves as the uniquely colored neighbor for $g_i$. 
%Along the path of length $4p$, 
%every fourth vertex is colored starting from the initial colored vertices ($\{d_i,e_i\}$ or $\{e_i,f_i\}$). 
%%%%%



\textcolor{red}{Now, all that remains to show is that $G(\phi)$ is a planar unit disk intersection graph.} 


%We now show that the unit disk intersection graph $G(\phi)$ is \cfonp{} colorable using one color if and only if $\phi$ is 1-in-3-satisfiable. 
%For the forward direction, let $C$ be a \cfonp{} coloring of $G(\phi)$ using one color. Since the clause vertex $c$ for each clause does not have the uniquely colored neighbor from within the gadget, exactly one of its neighbors $d_1,d_2,d_3$ is colored and this ensures that exactly one of the three variable gadgets have the vertices $a_{j\ell}$ and $b_{j\ell}$ colored. Therefore we get that the corresponding variable in $\phi$ is set to true. 

%For the reverse direction, let $\phi$ have a 1-in-3-satisfying assignment. For each of the variables that are true in $\phi$, their corresponding true vertices in variable gadgets are colored. For variables that are not true in $\phi$, all the vertices other than the true vertices in the gadget are colored. 
%This coloring can be extended to the vertices along the path that connects the clause gadget and the variable gadget to be \cfonp{} coloring using one color. The coloring also ensures that the clause vertex has a uniquely colored vertex. 



\qed
\end{proof}

==> Unused/unitsquareanddisk-app.tex <==
\section{Proof of Theorem \ref{thm:unitdisk} }\label{app:unitdisk}



%\subsection{Proof of Theorem \ref{thm:unitdisk}}
Each disk is identified by its center. By unit disk, we mean that its radius is 1. 
%the distance between its center and its sides is 1 i.e., length of each side is 2. 
Sometimes we interchangeably use the term ``vertex'' for unit disk.
% We first show that two colors are sufficient to \cfonp{} color unit disk
% intersection graphs of height at most $\sqrt{3}$.
%A stripe is the region between two horizontal lines of infinite length. 
We consider a unit disk as belonging to a stripe 
if its center is contained in the stripe. 
If a unit disk has its center on the horizontal line that separates two stripes 
then it is considered in the stripe below the line. 

%The bottom most stripe is identified as the region between the horizontal line passing through center of the unit square with the least Y-coordinate and another horizontal line at height 2 from existing horizontal line. 
We say that a unit disk intersection graph has \emph{height $\sqrt{3}$}, if 
the centers of all the disks lie in a horizontal stripe of width $\sqrt{3}$.
% We first prove that 
%two colors are sufficient to \cfonp{} color all the unit disk intersection graphs of height $\sqrt{3}$.
%The approach for the general case  
%to arriving at the bound 
is to divide the graph into horizontal stripes of height $\sqrt{3}$ and color
the vertices in two phases. 
Throughout, we denote the $X$-coordinate and the $Y$-coordinate of a vertex $v$ with $v_x$ and $v_y$ respectively. 
%We first prove %in 
%Lemma \ref{lem:unit_sq_heig2} 
%that, for all unit square intersection graphs $G$ of height 2, 
%(i.e., the centers of all squares lie in a horizontal stripe of height 2), 
%two colors are sufficient to \cfonp{} color $G$. 
%This result is extended to get a bound for a general unit intersection graph. 
%in Lemma \ref{lem:unit_sq_ub}. 

The proof of this theorem will be similar to the proof of Theorem \ref{thm:unit_sq_ub},
but different in the following three aspects: 

\begin{itemize}
    \item In Theorem \ref{thm:unit_sq_ub}, we used the result that unit square graphs
of height 2 are CFON$^*$ 2-colorable. In this theorem, we will use the result that
unit disk intersection graphs of height $\sqrt{3}$ are \cfcnp{} 2-colorable, and not 
\cfonp{} 2-colorable.

    \item In Theorem \ref{thm:unit_sq_ub}, the set $I$ for which we needed to identify 
    the uniquely colored neighbor was the set of isolated vertices in the respective stripe.
    In this theorem, the set $I$ will be the set of vertices colored in phase 1.
    
    \item In Theorem \ref{thm:unit_sq_ub}, the phase 2 coloring involved considering the representative
    vertices in the order of their $X$-coordinate. For the phase 2 coloring of this theorem,
    we consider the vertices in $I$ in the order of their $X$-coordinate and then color the 
    representative vertices.
\end{itemize}


We will use the following lemma from \cite{Sandor2017}.

\begin{lemma}{\cite[Theorem 7]{Sandor2017}}
\label{lem:disk_sqrt3}
Unit disk intersection graphs of height~$\sqrt{3}$ are \cfcnp{} 2-colorable.
Further, the horizontal distance between two colored vertices is greater than 1.
\end{lemma}

Note that the above lemma pertains to CFCN$^*$ coloring and not CFON$^*$ coloring. The second sentence in the above lemma is not stated in the statement of Theorem 5 in \cite{Sandor2017}, but rather in its proof. We will use the CFCN$^*$ coloring used in the above stated lemma in the process of arriving at a CFON$^*$ bound for unit disk intersection graphs. Below we reproduce the coloring process
used in the proof of the above lemma in \cite{Sandor2017}.


\begin{proof}[Coloring process used in Lemma \ref{lem:disk_sqrt3}]
Let $G=(V,E)$ be a unit disk intersection graph such that
the centers of all the disks in $G$ lie in a band of height $\sqrt{3}$. 
The vertices $V(G)$ are processed according to their non-decreasing $X$-coordinate. 
At each step of the algorithm, we choose a vertex $v$ that covers all uncolored vertices to its left, and assign the color 1 (or 2) if the previous colored vertex was assigned the color 2 (or 1). A vertex $v$ is \emph{covered} if and only if either it is colored or has a neighbor  assigned 
a color from $\{1, 2\}$. At the end, each uncolored vertex is assigned the color 0. 
It follows from the algorithm that the horizontal distance between any two colored vertices is greater than 1. 
The reader is directed to \cite{Sandor2017} for the correctness of the algorithm. 
\qed
\end{proof}


We assign colors 
$C(v)$, 
for all the unit disks $v$ of $G$ in two phases.
In phase 1, we use 6 non-zero colors 
$C: V \to \{0\} \cup \{c_{i,0}, c_{i,1} \mid  i \in \{0,1,2\}\}$. 
WLOG we assume that the centers of all the disks have positive $Y$-coordinates.
We partition the plane into horizontal stripes $S_{\ell}$ for $\ell \in \mathbb{N}$
where each stripe is of height $\sqrt{3}$. 
We assign vertex $v$ with $Y$-coordinate $v_y$ to $S_{\ell}$ if $\sqrt{3}(\ell-1) < v_y \leq \sqrt{3}\ell$. 
Then $G[S_\ell]$ has height $\sqrt{3}$.
\hhcomment{Did we define $G[S_\ell]$ before?}
We \cfcnp{} color vertices in $S_{\ell}$ accordingly using colors $c_{i,0}, c_{i,1}$ where $i = \ell \bmod 3$, by Lemma~\ref{lem:disk_sqrt3}.
Let $I$ be the set of all colored vertices after this phase.
Our goal is to \cfonp{} color all the vertices. 
Any vertex not in $I$ has a uniquely colored neighbor that is not itself (after phase 1), 
and hence we need
to identify uniquely colored neighbors for vertices in $I$.
%We will show later on that any vertex not in $I$ has a uniquely colored neighbor in $G$.

In phase 2, we will reassign colors to some vertices of $G$ to ensure a uniquely colored neighbor for each vertex in $I$.
For each vertex $v\in I$, choose an arbitrary \textit{representative vertex} $r(v)\in N(v)$.
%\skcomment{What if such a representative does not exist? Can we claim that $v$ already has 
%a uniquely colored neighbor? I checked the proof in Fekete Keldenich, and they 
%don't rule out a colored vertex seeing two other vertices of the same color-- THIS ISSUE NEEDS TO BE FIXED}
Note that two vertices in $I$ may share the same representative vertex.
% Let $I_1$ and $I_2$ be the vertices in $I$ that are colored $c_{i,0}$ and $c_{i,1}$, respectively, for $i \in \{0, 1, 2, 3\}$.
Let $R = \{r(v) \mid v \in I\}$ be the set of representative vertices.
We assign $C': R \to \{c'_{i,j} \mid  i \in \{0,1,2,3,4,5\}, j \in \{0,1, \ldots, 7\} \}$.
Consider a stripe $S_{\ell}$ for $\ell \in \mathbb{N}$.
We order the vertices $S_{\ell} \cap I$ non-decreasingly by their $X$-coordinate.
We consider the vertices sequentially in that order. 
If the representative vertex of the current vertex has not yet been colored in phase 2, we color the representative vertex with a color in $\{c'_{i,0},\dots,c'_{i,7} \mid i \equiv \ell \bmod 6 \}$ in a cyclic manner (i.e., the first vertex to be colored will take color $c'_{i,0}$, and the next $c'_{i,7}$, and so on). Notice that we consider the vertices as per the order in $S_{\ell} \cap I$, and not as per 
the order in $S_{\ell} \cap R$.

\noindent
\textbf{Total number of colors used:} The number of colors used in phase 1 and phase 2 are 6 and 48 respectively, giving a total of 54.

\noindent
\textbf{Correctness:} 
We now prove that the assigned coloring is a valid \cfonp{} coloring, by showing that every vertex has a uniquely colored neighbor.

Firstly, we consider a vertex~$v$ not in~$I$ and in $G[S_\ell]$ for some $\ell$.
By definition of the set~$I$, $v$ is adjacent to a vertex~$u$ color by $C$, after the phase 1.
Suppose $u$ is not recolored in phase 2.
Then since~$C$ is a \cfcnp{} coloring of $G[S_{\ell}]$, $v$ is adjacent to a uniquely colored neighbor~$u \neq v$ in $G[S_\ell]$.
By the coloring, the distance between $v$ and other vertices in another stripe with the same coloring as $u$ is at least $2\sqrt{3} > 2$.
%\skcomment{I suppose the previous sentence follows from 
%the correctness of the CFCN* coloring. We can either mention this, 
%or skip it (as it is evident from the fact that C is a CFCN* coloring.}
Hence, $u$ is the uniquely colored neighbor of~$v$ in~$G$.

Now suppose $u$ is recolored in phase 2 to some color $c'_{i,j}$.
For the sake of contradiction, suppose that~$v$ is also adjacent to another vertex~$w$ with the same color~$c'_{i,j}$.
Then~$u$ and~$w$ must be the representative vertices of two vertices~$a$ and~$b$ in $I$ that are in stripes $S_{\ell}$ and $S_{\ell'}$, respectively, such that $\ell \equiv \ell' \bmod 6$.
Since $(a,u,v,w,b)$ forms a path in $G$, and since two adjacent vertices in $G$ have Euclidean distance at most 2, we conclude that $a$ and $b$ are at the distance of at most 8.
If $\ell \neq \ell'$, then $|\ell - \ell'| \geq 6$.
This implies $|a_y - b_y| \geq 5\sqrt{3} > 8$, a contradiction.
Hence, $a$ and $b$ are in the same stripe.
Because $u$ and $w$ have the same color, there must be 7 other vertices in $I$ between $a$ and $b$ in terms of the $X$-coordinate.
By Lemma~\ref{lem:disk_sqrt3}, this implies $|a_x - b_x| > 8$, another contradiction.
Hence, $v$ cannot be adjacent to two vertices of the same color.

%\skcomment{I think we need to argue that $u$ and $w$ are also in the same stripe. This follows easily %from $u, w$ being common neighbors of $v$ and hence distance between $u$ and $w$ is at most 4. Since 
%we repeat colors in groups of 4, this implies that $u, w$ have to be 
%in the same stripe. Else $|u_y - w_y| > 3\sqrt{3} > 5$.
%Second, in the case when $a$ and $b$ are in the same stripe, we can 
%talk about $u$ and $w$ being colored with the same color. 
%This means that $|u_x - w_x| > 8$. But this contradicts the fact that
%distance between $u$ and $w$ is at most 4. 
%We may be able to bring down the number of distinct stripes to 4, 
%and colors per stripe to 5 (or 4).
%}


Lastly, we consider a vertex~$v$ in $I$.
Then the representative~$u$ of~$v$ is colored by $C'$.
With the same argument as above, we can conclude that~$v$ is not adjacent to another vertex with the same color.


\begin{comment}

We assign colors 
$C(v)$, 
for all the unit disks $v$ of $G$ in two phases.
In phase 1, we use 6 colors 
$C: V \to \{0\} \cup \{c_{i,0}, c_{i,1}, c_{i,2} \mid  i \in \{0,1,2\}\}$. 
%$\{ c_{i,0}, c_{i,1} \mid i \in \{0,1,2\} \}$.
WLOG we assume that the centers of all the disks have positive $Y$-coordinates.
We partition the plane into horizontal stripes $S_{\ell}$ for $\ell \in \mathbb{N}$
where each stripe is of height $\sqrt{3}$. 
We assign vertex $v$ with $Y$-coordinate $v_y$ to $S_{\ell}$ if $\sqrt{3}(\ell-1) < v_y \leq \sqrt{3}\ell$. 
\textcolor{red}{Then $G[S_\ell]$ has height $\sqrt{3}$ such that Lemma \ref{lem:unit_sq_heig2} applies.}
We color vertices in $S_{\ell}$ accordingly using colors \bscomment{$c_{i,0}$, $c_{i,1}$ and $c_{i,2}$} where $i = \ell \bmod 3$.
Then every vertex $u \in S_{\ell}$, that is not isolated in $G[S_{\ell}]$ has a uniquely colored neighbor $v$ in $G[S_{\ell}]$.
Every $w \notin S_{\ell}$ with color $C(w)=C(v)$ must be in a stripe $S_{\ell^\star}$ with $|\ell-\ell^\star|\geq 3$.
Thus $w \notin N(u)$ and $v$ is also a uniquely colored neighbor of $u$ in $G$.
%
It remains to identify uniquely colored neighbors for the vertices $u \in S_\ell$ 
%for $i \in \mathbb{N}$ 
which are isolated in $G[S_{\ell}]$.
Let $I$ be the set of these vertices.

%It remains to ensure that a uniquely colored neighbor for the vertices $u \in S_\ell$ 
%for $i \in \mathbb{N}$ 
%which are isolated in $G[S_{\ell}]$.
%Let $I$ be the set of those vertices.

In phase 2, we reassign colors to some of the vertices of $G$ to ensure a uniquely colored neighbor for each vertex in $I$.
For each vertex $v\in I$, choose an arbitrary \textit{representative} vertex $r(v)\in N(v)$.
Let $R = \{r(v) \mid v \in I\}\subseteq V(G)$ be the set of representative vertices.
We assign $C: R \to \{c_{i,j} \mid  i \in \{0,1,2\}, j \in \{3, 4, \ldots, 17\} \}$
    that replaces the color assigned in phase 1.
Consider a stripe $S_{\ell}$ for $\ell \in \mathbb{N}$.
We order the vertices $S_{\ell} \cap R$ non-decreasingly by their $X$-coordinate and
    sequentially color them with $c_{i,3},\dots,c_{i,17}$ where $i = \ell \bmod 3$. 
    
\noindent
\textbf{Total number of colors used:} The number of colors used in phase 1 and phase 2 are 9 and 45 respectively, giving a total of 54.




\noindent
\textbf{Correctness:} 
%Let $G=(V,E)$ be the unit square intersection graph. After the phase 1 coloring, let $I$ denote the set of vertices for which there exists no uniquely colored neighbor. 
%For each vertex $v\in I$, we chose a representative vertex $r_v$. Let the set of representative vertices of $I$ be denoted by the set $R$. 
%In order words, $I$ is the set of vertices participating in phase 2 coloring. 
We now prove that the assigned coloring is a valid \cfonp{} coloring. For this we need to prove the following, 
\begin{itemize}
    \item Each vertex in $I$ has a uniquely colored neighbor. 
    
    \item The coloring in phase 2 does not upset the uniquely colored neighbors (identified in phase 1) of the vertices in $V\setminus I$. 
\end{itemize}

We first prove the following claim. 

\begin{claim}
%Let $G$ be a unit square intersection graph. 
For each vertex $v\in V(G)$, all vertices in $N(v) \cap R$ are assigned distinct colors in phase 2.
%if there exists a vertex  $u\in N(v)$ such that $|$C(u)$\cap \{c_1, \dots, c_{21}\}|=1$, then $C(u)\neq C(w)$, for each $w\in N(v)\setminus u$. 
\end{claim}
\begin{proof}[Claim's proof]
Let $v \in S_{\ell+1}$.
Assume, for the sake of contradiction, that there are two vertices $u, w\in N(v) \cap R$ such that $C(u)=C(w)$, see also Figure \ref{fig:unitdisk}.
Then $u$ and $w$ have to be from the same stripe that neighbors $S_{\ell +1}$.
%\thcomment{a common stripe which neighbors $S_{\ell+1}$} 
%a neighboring stripe 
WLOG let $u, w\in S_\ell$, $\ell=0 \bmod 3$ and $u_x \leq w_x$. 
We may further assume that $C(u) = C(w) = c_{0,3}$.
Then there are sixteen vertices (including $u$ and $w$) $R' \subseteq R \cap S_\ell$ that are assigned the colors $c_{0,3},c_{0,4},\dots, c_{0,17}, c_{0,3}$ and have $X$-coordinate between $u_x$ and $w_x$.
Note that $|u_x - v_x| < 2$ and $|w_x - v_x| < 2$. This is because of the fact that $v\in S_{\ell+1}$, 
$u,w,\in S_{\ell}$ and $u,w\in N(v)$. 
This implies that $|u_x- w_x|<4$. 
Vertices $R'$ are the representative vertices of some sixteen vertices ${I}' \subseteq I$.
By definition $I' \subseteq S_{\ell+1} \cup S_{\ell-1}$. Before we proceed to the rest of the proof, we observe the following.
%, the proof of which is intuitive.

\medskip

\noindent
\textbf{Observation:} Let $p,q$ be vertices in a stripe $S$. If $p\notin N(q)$, then $|p_x - q_x | > 1$. 
\begin{proof}
Note that $|q_y - p_y|< \sqrt{3}$ since $p$ and $q$ belong to the same stripe $S$.
Because $p$ and $q$ are non-adjacent,
    they have Euclidean distance of more than $2$.
Then if follows that $|p_x - q_x | > 1$.
%When $p\notin N(q)$, the minimum value of $|p_x-q_x|$ is obtained when they are as close as possible. 
%We claim that $|p_x-q_x|>1$. 
%If  $|p_x-q_x|\leq1$, we get that $p$ and $q$ are adjacent, which is a contradiction to the assumption. Hence $|p_x-q_x|>1$. 
%When $|p_x-q_x|>1$, $p$ and $q$ could intersect at one point. This happens when $p$ and $q$ lies on the two horizontal stripes that defines the stripe $S$. 
%
%For $pq\in E(G)$, the distance between $p$ and $q$ is at most 2. This implies $|p_x-q_x|\leq 2$. $|p_x-q_x|$ is minimum when $p$ and $q$ lie on the horizontal line that defines the stripe $S$. 
%For $pq\notin E(G)$, the distance between $p$ and $q$ is at most 2. This implies $|p_x-q_x|\leq 2$. 
%If their distance is 2, $|p_x-q_x|$ we say $p\in N(q)$ when $|p_x-q_x|\leq 2$. 
%when This implies $|p_x - q_x|\leq 2$. 
%For $pq\notin E(G)$, We now look at the scenario when $|p_x-q_x|$ is minimum when condition when The vertices $p$ and $q$ have distance 2, are closet when can be is when Since each stripe is of height $\sqrt{3}$, 
\qed
\end{proof}

First, let us consider $I' \cap S_{\ell+1}$.
We claim that there are at most three vertices $u',u'', u''' \in {I}' \cap S_{\ell+1}$ 
such that $u'_x, u''_x, u'''_x < v_x$. 
%$u'_x < v_x$,  $u''_x<v_x$ 
%and $u'''_x<v_x$ \thcomment{$u_x',u_x'',u_x'' < v_x$}. %with a lower $X$-coordinate than $v$. 
WLOG let $u'''_x< u''_x < u_x <u'_x$. 
By the above observation, we have $|u'_x - v_x| >1$, $|u''_x - v_x| > 2$ and $|u'''_x - v_x| > 3$. 
%\thcomment{only if we assume some ordering}.
 For the sake of contradiction, assume that there is another vertex $u^\star \in {I}' \cap S_{\ell+1}$ such that $u^\star_x 
< v_x$. WLOG let $u^\star_x< u'''_x$. 
Since $u^\star\in {I}' \cap S_{\ell+1}$, it should be the case that $|u^\star_x - u_x|\leq 2$. This is not the case because $|u^\star_x - v_x|>4$ and $|v_x - u_x|<2$ implying $|u^\star_x - u_x|>2$. 
%Analogously, there is at most one vertex $w' \in {I}' \cap S_{\ell+1}$ such that $w'_x > v_x$.
%Considering the possibility that $v \in I'$, we have $|I' \cap S_{\ell+1}|\leq 3$.
Analogously, there are at most three vertices $w', w'',w''' \in {I}' \cap S_{\ell+1}$ such that $w'''_x, w''_x, w'_x > v_x$.
Considering the possibility that $v \in I'$, we have $|I' \cap S_{\ell+1}|\leq 7$. %\thcomment{not compatible with the second last sentence}.

Now, consider the vertices in $I' \cap S_{\ell-1}$.
Again any vertex  in $I' \cap S_{\ell-1}$ must be adjacent to some representative $r \in R'$ with $|r_x-v_x| < 2$.
Thus the $X$-coordinates of the vertices in $I' \cap S_{\ell-1}$ differ by at most 8.
Since the vertices in $I' \cap S_{\ell-1}$ are non-adjacent, we have that $|I' \cap S_{\ell-1}|\leq 8$. 
Together with the vertices in $I'\cap S_{\ell+1}$, we have that $|I'|=15$. 
This contradicts the assumption that $|I'| = 16$. 
Thus all vertices $N(v) \cap R$ are assigned distinct colors.
\qed
\end{proof}

We now proceed to the correctness part. 
\begin{itemize}
    \item 
\textbf{Every vertex $v\in I$ has a uniquely colored neighbor.} 

Let $v\in S_{\ell+1} \cap I$. 
%be an isolated vertex in stripe $S_{i-1}$ 
%and $r_v$ be its representative vertex in $S_i$. 
%The vertex $r_v$ is the uniquely colored neighbor for $v$. 
By the above claim, no two vertices in $N(v) \cap R$ are assigned
the same color in phase 2.
Moreover, since $v$ is not isolated in $G$, we have $|N(v) \cap R|\geq 1$ such that it has a uniquely colored neighbor.


%\noindent
\item \textbf{The coloring in phase 2 does not upset the uniquely colored neighbors of vertices in $V\setminus I$.} 

Let $v\in V\setminus I$ and $u$ be its uniquely colored neighbor after the phase 1 coloring. 
For $v$ to not have a uniquely colored neighbor after phase 2 coloring, 
there exists a vertex $w\in N(v)$ such that $C(u)=C(w)$. 
This implies that both $u$ and $w$ are representative vertices for some vertices in 
$I$ and they are re-colored in phase 2.
This contradicts the above claim.
%By the above claim, it can not happen that $C(u)=C(w)$ where $C(u)\in \{c_1,\cdots, c_{21}\}$. 
\end{itemize}
\qed



\begin{figure}[t!]
\centering
\begin{tikzpicture}[every node/.style={node distance=1.8cm,scale=0.9}, scale = 0.5]

\tikzstyle{vertex}=[dot, draw, minimum size=8pt]
\draw[gray] (-6,2.4) -- (7,2.4);
\draw[gray] (-6,0.4) -- (7,0.4);


\draw[thick, thin] (5,3) circle (1cm);
%draw[thick, thin] (4,2) circle (6,4); 
\draw[thick, thin] (3.7,-0.8)  circle (1cm);
\draw[thick, thin] (1.5,-0.8)  circle (1cm);
\draw[thick, thin] (-0.7,-0.8)  circle (1cm); 
\draw[thick, thin] (-2.9,-1.8)  circle (1cm);
\draw[thick, thin] (-3,3)  circle (1cm);
\draw[black, double=black] (2.5,1.2)  circle (1cm); 
\draw[black, double=black] (-0.5,1.2)  circle (1cm); 
\draw[black, double=black] (1,2.6)  circle (1cm);
%\draw[orange, thick, dotted] (-1,-4) -- (-1,6);
%\draw[orange, thick, dotted] (3,-4) -- (3,6); 

\node at (1.2,2.6) {$v$};
%\node[above, blue]  at (5,4) {$u_2$};
\node at (2.5,1.2) {$w$};
\node  at (-0.5,1.2) {$u$}; 
\node at (-6,4) {$S_{\ell+1}$};
\node at (-6,-1) {$S_{\ell-1}$}; 
\node at (-6.2, 1.4) {$S_\ell$}; 

%\node[above, blue] at (-3, 4) {$u_1$}; 
%\node[below, blue] at (-3, -2) {$u_3$}; 
%\node[below, blue] at (-0.6, -2) {$u_4$};
%\node[below, blue] at (1.4, -2) {$u_5$};
%\node[below, blue] at (3.6, -2) {$u_6$};


%\node[draw, red]  at (-1,-7.5) {u};

%\node[draw, red]  at (-10,-8) {Colors $\{4,5,6\}$};
%\node[draw, black]  at (-10,-4) {Colors $\{7,8,9\}$};
%\node[draw, blue]  at (-10,0) {Colors $\{1,2,3\}$};
%\node[draw, black]  at (-10,4) {Colors $\{4,5,6\}$};
%\node[draw, black]  at (-10,8) {Colors $\{7,8,9\}$};



\end{tikzpicture}
\caption{The vertex $v$ The figure describes the neighborhood of isolated vertices 
%around an isolated vertex $v$ 
in the stripes $S_{\ell+1}$, $S_\ell$ and $S_{\ell-1}$ around the representative vertices $u$ and $w$ (marked in black). 
%depicts the isolated vertices participating in phase 2. 
The isolated vertices participating in phase 2 coloring are colored in blue and $v$ is the vertex under consideration.  
%while 
%The representative vertices $u$ and $w$ are marked in black. 
Each stripe is of height 2 and the separation line of two stripes is marked in green. 
%The stripe $S_i$ under consideration is of height 2 and the region is between the lines marked in green. 
%There are six other representative vertices between the dashed lines in $S$. 
%The isolated vertex $v$ for which 
}
\label{fig:unitdisk}
\end{figure}
\end{comment}





\begin{lemma}\label{lem:unit_disk_heig2}
Unit disk intersection graphs of height $\sqrt{3}$ are \cfonp{} 5-colorable. 
\end{lemma}
\begin{proof}

% We order the disks by their centers lexicographically, that is, for two disks $D$ and $D'$, $D \prec D'$ if $D_x < D'_x$ or $D_x = D'_x$ and $D_y < D'_y$.
We assign colors $f:\mathcal I\rightarrow \{1, 2, 3, 4, 5, 0\}$ to all the disks in the stripe of height $\sqrt{3}$. 
We assign the colors 1, 2, 3, 4 and 5 to vertices in this order, one in each iteration $1\leq j \leq \ell$. 
We start with a disk $v^1$ that is the smallest in the order and assign $f(v^1)=1$. 
For $j\geq 2$, we do the following. 
Choose a disk $v^j\in N(v^{j-1})$ such that  
(i) there exists an uncolored disk $w\in N(v^j)\setminus N(v^{j-1})$, and 
(ii) $u_x < v^{j}_x$ for all $u\in N(v^{j-1})$ that satisfies (i). 
In case of multiple such $v^j$, choose a $v^j$ such that $w_x$ of its uncolored neighbor $w$  is the largest. 
For all the uncolored disks $u$ where $u_x \leq v^j_x$,
% or $u \in N(v^j)$, 
we assign $f(u)=0$. We stop at the disk $v^{\ell}$ 
if $v^{\ell}$ has no neighbor satisfying condition (i).
For the iterations 2, 3, 4 and 5, we assign $f(v^2)=2, f(v^3)=3$, $f(v^4)=4$ and $f(v^5)=5$. For all other iterations where $j\geq 6$, 
we assign $f(v^j)=\{1, 2, 3, 4, 5\}\setminus \{f(v^{j-1}), f(v^{j-2}), f(v^{j-3}), f(v^{j-4})\}$. 

Before we proceed to the correctness of the algorithm, we first observe the following. 
\begin{claim}\label{obs:ud4}
In any coloring $f$, there exists at most two non-zero colored vertices $u, v$ such that $u_x=v_x$. 
\end{claim}
\begin{proof}
Suppose there are three non-zero colored vertices $u,v$ and $w$ such that $u_x=v_x=w_x$. %WLOG let $f(u)=1, f(v)=2$ and $f(w)=3$. 
The above algorithm chooses vertices to be colored in a 
such way that the $X$-coordinate of the colored vertices are
non-decreasing.
\hhcomment{Why?}
Hence WLOG, we may assume that the algorithm colored the vertices $u$, $v$ and $w$ in successive iterations in this order.
%If not, we select the three vertices that were chosen successively by the algorithm as $u$, $v$ and $w$.
So vertices $v$ and $w$ are chosen by the vertices $u$ and $v$ respectively, according to the coloring rules. 

There are two reasons why $w$ was not chosen by $u$: either $w$ had no uncolored neighbor in $N(w)\setminus N(u)$ or 
%there exists vertices $v'$ and $$both $v$ and $w$ had uncolored neighbors in $N(v)\setminus N(u)$  and $N(w)\setminus N(u)$ respectively and that 
$v'_x\geq w'_x$, where $v'$ and $w'$ are the uncolored neighbors in $N(v)\setminus N(u)$  and $N(w)\setminus N(u)$ respectively. 
% \hhcomment{Why are $v'$ and $w'$ involved here? Maybe we should have a lexicographical order of the vertices and choose the largest among the eligible neighbours of $u_x$, then this case cannot happen.}
%or  
The former case is not possible as then $w$ does not satisfy (i) to be chosen after coloring $v$. 
In the latter case, there exists a vertex $v'$ and the algorithm would pick $v'$ instead of $w$ according to the rules. 
\qed
\end{proof}

If the algorithm had chosen three colored
%If the algorithm picked two colored 
disks $v^{j-1}$, $v^j$ and $v^{j+1}$, then it follows that 
$v^{j+1} \notin N(v^{j-1})$. Else the algorithm would have
chosen $v^{j+1}$ instead of $v^j$ in the $j$-th iteration.
Since the height of the stripe is $\sqrt 3$, 
we have that $v^{j+1}_x-v^{j-1}_x>1$. 
Thus any two vertices $u,v$ assigned the same color from $\{1, 2, 3, 4, 5\}$ have $|u_x-v_x|>2$. 
Hence vertices assigned the same color do not intersect with each other. 
\hhcomment{Why is this important?}

Vertex $v^j$ is adjacent to $v^{j+1}$ for $1\leq j\leq \ell -1$. 
% For $v^{\ell}$, the uniquely colored neighbor is $v^{\ell -1}$. 
% Recall that the vertex $v^j$ is picked in the $j$-th iteration because $v^j$ has an uncolored neighbor.  
Note that the vertices $v^{j-4}$ and $v^{j+6}$ share the same color as $v_{j+1}$.
From the above observation, $|v^{j}_x-v^{j-2}_x|>1$ and $|v^{j-2}_x-v^{j-4}_x|>1$. Therefore $|v^{j}_x-v^{j-4}_x|>2$.
Similarly, $|v^{j}_x-v^{j+6}_x|>2$. 
%We now have to show that $v^{j-3}, v^{j+5}\notin N(v^{j})$. Note that the vertices $v^{j-3}, v^{j+1}$ and $v^{j+5}$ are assigned the same color. Since $|v^{j}_x-v^{j+4}_x|>2$, we have that $|v^{j}_x-v^{j+5}_x|>2$. Suppose $v^{j-3}\in N(v^j)$. 
%The only reason $v^{j-3}$ did not pick $v_j$ instead of $v^{j-2}$ should be that $v^{j-2}_x=v^{j-1}_x=v^{j}_x$. But this is not possible according to the above claim. 
Hence, $v^{j+1}$ is a uniquely colored neighbor of $v^{j}$. 
%Then the vertex $v^{j-3}$ would have chosen $v_j$ as $v^{j-2}$ because $v^{j}_x\geq v^{j-1}_x\geq v^{j-2}_x$ and the above claim. 
%Note that $v^{j-2}_x$

By a similar argument, we note that the last vertex colored by
the algorithm, $v^{\ell}$, is adjacent to $v^{\ell -1}$ and not $v^{\ell -6}$. Hence $v^{\ell -1}$ is the uniquely colored neighbor of $v^{\ell}$.

The vertices assigned the color 0 also have a uniquely colored neighbor. For each $v$ such that $f(v)=0$ and $v^{j}_x\leq v_x \leq v^{j+1}_x$, for some $j$, it is the case that $v\in N(v^j)\cup N(v^{j+1})$. 
This is because $|v^{j+1}_x-v^{j}_x|\leq 2$. Hence it follows that
either $|v^{j+1}_x-v_x|\leq 1$ or $|v^{j}_x-v_x|\leq 1$. 
WLOG, let $|v^{j}_x-v_x|\leq 1$. 
Then we claim that $v^j$ is the uniquely colored neighbor of $v$. 
For $v$ to not have $v^j$ as a uniquely colored neighbor, it should be the case that either $v^{j+5}\in N(v)$ or $v^{j-5}\in N(v)$. 
Since $v^j_x\leq v_x$ and $|v^j_x-v^{j-5}_x|>2 $, we have that $|v_x-v^{j-5}_x|>2 $ and $v^{j-5}\notin N(v)$. 
Similarly, since $v_x\leq v^{j+1}_x$ and $|v^{j+1}_x-v^{j+5}_x|>2$, we have that $|v_x-v^{j+5}_x|>2$ and $v^{j+5}\notin N(v)$. 
\qed
\end{proof}

%\textbf{Remark:} 

%Since all the vertices 
%are in a stripe of height $\sqrt 3$, it follows that 
%$v^j \in N(v)$.
%a colored neighbor $v^j$ such that $f(v^j)=1$. 
%We claim that $v_j$ is the uniquely colored neighbor for $v$. 
%For $v$ to not have $v^j$ as a uniquely colored neighbor, it should be the case that either $v^{j+4}\in N(v)$ or $v^{j-4}\in N(v)$. 
%Since $|v^{j}_x-v^{j-4}_x|\geq 2$, we have that $|v_x-v^{j-4}_x|\geq 2$ and therefore $v^{j-4}\notin N(v)$. 
%Suppose $v^j,v^{j+4}\in N(v)$. 
%The reason for $v^j$ choosing $v^{j+1}$ over $v$ in the $j+1$-th iteration may be because of the following three cases. Let $w^{j+1}$ (resp. $w$) be the uncolored neighbor of $v^{j+1}$ (resp. $v$) with the largest $x$-coordinate among its uncolored neighbors. Since $v^{j+4}\in N(v)$, it is clear that the vertex $w$ exists. 

%Note that $w=v^{j+4}$ because of our assumption. Note that  a vertex which has greater $x$-coordinate that $v^{j+4}$ is a candidate for $w$. 
%For the sake of simplicity, we may consider $w=v^{j+4}$. 

%Notice that since $v^{j+4} \in N(v)$, we have that  $w_x \geq v_x^{j+4}$.


%\begin{itemize}
%    \item \textbf{Case 1:} $v^{j+1}_x=v_x$ and $w^{j+1}_x=w_x$
    
%    Note that $w_x^{j+1}\geq v_x^{j+2}$. This $v^{j+2}_x=v^{j+4}_x$. This is not possible because $|v^{j+2}_x-v^{j+4}_x|>1$. 

%    \item \textbf{Case 2:} $v^{j+1}_x=v_x$ and $w^{j+1}_x>w_x$
    
%    Note that $w^{j+1}=v^{j+2}$. This implies that $v^{j+2}_x>v^{j+4}_x$ which is not possible because the algorithm picks the colored vertices such that their $x$-coordinates are non-decreasing. 
%    \item \textbf{Case 3:} $v^{j+1}_x>v_x$
    
%    It is clear that $v^{j}_x<v_x<v^{j+1}_x$. We now argue based on whether $v^{j+1}\in N(v^{j+4})$ or not. 
%    If $v^{j+1}\in N(v^{j+4})$, then similar to the above cases, $v^{j+4}$ would have been the $v^{j+3}$. 
%    Else if $v^{j+1}\notin N(v^{j+4})$, 
%\end{itemize}

%because if a vertex is adjacent to two vertices assigned the color 1, then it is adjacent to at least two colored vertices, the color of which appears exactly once in its neighborhood. Also every colored vertex will have a uniquely colored neighbor.  



%\textcolor{red}{
%\begin{lemma}
%Unit disk intersection graphs of height $\sqrt{3}$ are \cfonp{} 4-colorable. 
%\end{lemma}
%\begin{proof}
%Let $G$ be a unit disk intersection graph of height $\sqrt{3}$.
%Note that vertices $u$ and $v$ are adjacent if and only if their $X$-coordinates differ by at most $2$.
%\hhcomment{The above statement is wrong.} 
%Thus we may represent $G$ as a unit interval graph by replacing every vertex $v$ 
%$X$-coordinate $x_v$ 
%by an interval from $v_x-1$ to $v_x+1$.
%Then $\chionp \leq 2$ as seen in Lemma \ref{lem:non_contained_interval}.
%
%\end{proof}
%}


We assign colors 
$C(v)$, 
for all the unit disks $v$ of $G$ in two phases.
In phase 1, we use 20 non-zero colors 
$C: V \to \{0\} \cup \{c_{i,0}, c_{i,1}, c_{i,2}, c_{i,3}, c_{i,4} \mid  i \in \{0,1,2,3\}\}$. 
%$\{ c_{i,0}, c_{i,1} \mid i \in \{0,1,2\} \}$.
WLOG we assume that the centers of all the disks have positive $Y$-coordinates.
We partition the plane into horizontal stripes $S_{\ell}$ for $\ell \in \mathbb{N}$
where each stripe is of height $\sqrt{3}$. 
We assign vertex $v$ with $Y$-coordinate $v_y$ to $S_{\ell}$ if $\sqrt{3}(\ell-1) < v_y \leq \sqrt{3}\ell$. 
Then $G[S_\ell]$ has height $\sqrt{3}$, by Lemma \ref{lem:unit_disk_heig2}.
We color vertices in $S_{\ell}$ accordingly using colors $c_{i,0}, c_{i,1}, c_{i,2}, c_{i,3}$ where $i = \ell \bmod 4$.
Then every vertex $u \in S_{\ell}$, that is not isolated in $G[S_{\ell}]$ has a uniquely colored neighbor $v$ in $G[S_{\ell}]$. %\bscomment{What does isolated mean ?}
Every $w \notin S_{\ell}$ with color $C(w)=C(v)$ must be in a stripe $S_{\ell^\star}$ with $|\ell-\ell^\star|\geq 4$.
Thus $w \notin N(u)$ and $v$ is also a uniquely colored neighbor of $u$ in $G$.
%
It remains to identify uniquely colored neighbors for the vertices $u \in S_\ell$ 
%for $i \in \mathbb{N}$ 
which are isolated in $G[S_{\ell}]$.
Let $I$ be the set of these vertices.

%It remains to ensure that a uniquely colored neighbor for the vertices $u \in S_\ell$ 
%for $i \in \mathbb{N}$ 
%which are isolated in $G[S_{\ell}]$.
%Let $I$ be the set of those vertices.

In phase 2, we reassign colors to some of the vertices of $G$ to ensure a uniquely colored neighbor for each vertex in $I$.
For each vertex $v\in I$, choose an arbitrary \textit{representative vertex} $r(v)\in N(v)$.
Let $R = \{r(v) \mid v \in I\}\subseteq V(G)$ be the set of representative vertices.
We assign $C: R \to \{c_{i,j} \mid  i \in \{0,1,2, 3\}, j \in \{5,6, \ldots, 19\} \}$
    that replaces the color assigned in phase 1.
Consider a stripe $S_{\ell}$ for $\ell \in \mathbb{N}$.
We order the vertices $S_{\ell} \cap R$ non-decreasingly by their $X$-coordinate and
    sequentially color them with $c_{i,5},\dots,c_{i,19}$ where $i = \ell \bmod 4$. 
    
\noindent
\textbf{Total number of colors used:} The number of colors used in phase 1 and phase 2 are 20 and 60 respectively, giving a total of 80.




\noindent
\textbf{Correctness:} 
%Let $G=(V,E)$ be the unit square intersection graph. After the phase 1 coloring, let $I$ denote the set of vertices for which there exists no uniquely colored neighbor. 
%For each vertex $v\in I$, we chose a representative vertex $r_v$. Let the set of representative vertices of $I$ be denoted by the set $R$. 
%In order words, $I$ is the set of vertices participating in phase 2 coloring. 
We now prove that the assigned coloring is a valid \cfonp{} coloring. For this we need to prove the following, 
\begin{itemize}
    \item Each vertex in $I$ has a uniquely colored neighbor. 
    
    \item The coloring in phase 2 does not upset the uniquely colored neighbors (identified in phase 1) of the vertices in $V\setminus I$. 
\end{itemize}

We first prove the following claim. 

\begin{claim}
%Let $G$ be a unit square intersection graph. 
For each vertex $v\in V(G)$, all vertices in $N(v) \cap R$ are assigned distinct colors in phase 2.
%if there exists a vertex  $u\in N(v)$ such that $|$C(u)$\cap \{c_1, \dots, c_{21}\}|=1$, then $C(u)\neq C(w)$, for each $w\in N(v)\setminus u$. 
\end{claim}
\begin{proof}[Claim's proof]
Let $v \in S_{\ell+1}$.
Assume, for the sake of contradiction, that there are two vertices $u, w\in N(v) \cap R$ such that $C(u)=C(w)$, see also Figure \ref{fig:unitdisk}.
Then $u$ and $w$ have to be from the same stripe that neighbors $S_{\ell +1}$.
%\thcomment{a common stripe which neighbors $S_{\ell+1}$} 
%a neighboring stripe 
WLOG let $u, w\in S_\ell$, $\ell=0 \bmod 4$ and $u_x \leq w_x$. 
We may further assume that $C(u) = C(w) = c_{0,5}$.
Then there are sixteen vertices (including $u$ and $w$) $R' \subseteq R \cap S_\ell$ that are assigned the colors $c_{0,5},c_{0,6},\dots, c_{0,19}, c_{0,5}$ and have $X$-coordinate between $u_x$ and $w_x$.
Note that $|u_x - v_x| < 2$ and $|w_x - v_x| < 2$. This is because of the fact that $v\in S_{\ell+1}$, 
$u,w,\in S_{\ell}$ and $u,w\in N(v)$. 
This implies that $|u_x- w_x|<4$. 
Vertices $R'$ are the representative vertices of some sixteen vertices ${I}' \subseteq I$.
By definition $I' \subseteq S_{\ell+1} \cup S_{\ell-1}$. Before we proceed to the rest of the proof, we observe the following.
%, the proof of which is intuitive.

\medskip

\noindent
\textbf{Observation:} Let $p,q$ be vertices in a stripe $S$. If $p\notin N(q)$, then $|p_x - q_x | > 1$. 
\begin{proof}
Note that $|q_y - p_y|< \sqrt{3}$ since $p$ and $q$ belong to the same stripe $S$.
Because $p$ and $q$ are non-adjacent,
    they have Euclidean distance of more than $2$.
Then if follows that $|p_x - q_x | > 1$.
%When $p\notin N(q)$, the minimum value of $|p_x-q_x|$ is obtained when they are as close as possible. 
%We claim that $|p_x-q_x|>1$. 
%If  $|p_x-q_x|\leq1$, we get that $p$ and $q$ are adjacent, which is a contradiction to the assumption. Hence $|p_x-q_x|>1$. 
%When $|p_x-q_x|>1$, $p$ and $q$ could intersect at one point. This happens when $p$ and $q$ lies on the two horizontal stripes that defines the stripe $S$. 
%
%For $pq\in E(G)$, the distance between $p$ and $q$ is at most 2. This implies $|p_x-q_x|\leq 2$. $|p_x-q_x|$ is minimum when $p$ and $q$ lie on the horizontal line that defines the stripe $S$. 
%For $pq\notin E(G)$, the distance between $p$ and $q$ is at most 2. This implies $|p_x-q_x|\leq 2$. 
%If their distance is 2, $|p_x-q_x|$ we say $p\in N(q)$ when $|p_x-q_x|\leq 2$. 
%when This implies $|p_x - q_x|\leq 2$. 
%For $pq\notin E(G)$, We now look at the scenario when $|p_x-q_x|$ is minimum when condition when The vertices $p$ and $q$ have distance 2, are closet when can be is when Since each stripe is of height $\sqrt{3}$, 
\qed
\end{proof}

First, let us consider $I' \cap S_{\ell+1}$.
We claim that there are at most three vertices $u',u'', u''' \in {I}' \cap S_{\ell+1}$ 
such that $u'_x, u''_x, u'''_x < v_x$. 
%$u'_x < v_x$,  $u''_x<v_x$ 
%and $u'''_x<v_x$ \thcomment{$u_x',u_x'',u_x'' < v_x$}. %with a lower $X$-coordinate than $v$. 
WLOG let $u'''_x< u''_x < u_x <u'_x$. 
By the above observation, we have $|u'_x - v_x| >1$, $|u''_x - v_x| > 2$ and $|u'''_x - v_x| > 3$. 
%\thcomment{only if we assume some ordering}.
 For the sake of contradiction, assume that there is another vertex $u^\star \in {I}' \cap S_{\ell+1}$ such that $u^\star_x 
< v_x$. WLOG let $u^\star_x< u'''_x$. 
Since $u^\star\in {I}' \cap S_{\ell+1}$, it should be the case that $|u^\star_x - u_x|\leq 2$. This is not the case because $|u^\star_x - v_x|>4$ and $|v_x - u_x|<2$ implying $|u^\star_x - u_x|>2$. 
%Analogously, there is at most one vertex $w' \in {I}' \cap S_{\ell+1}$ such that $w'_x > v_x$.
%Considering the possibility that $v \in I'$, we have $|I' \cap S_{\ell+1}|\leq 3$.
Analogously, there are at most three vertices $w', w'',w''' \in {I}' \cap S_{\ell+1}$ such that $w'''_x, w''_x, w'_x > v_x$.
Considering the possibility that $v \in I'$, we have $|I' \cap S_{\ell+1}|\leq 7$. %\thcomment{not compatible with the second last sentence}.

Now, consider the vertices in $I' \cap S_{\ell-1}$.
Again any vertex  in $I' \cap S_{\ell-1}$ must be adjacent to some representative $r \in R'$ with $|r_x-v_x| < 2$.
Thus the $X$-coordinates of the vertices in $I' \cap S_{\ell-1}$ differ by at most 8.
Since the vertices in $I' \cap S_{\ell-1}$ are non-adjacent, we have that $|I' \cap S_{\ell-1}|\leq 8$. 
Together with the vertices in $I'\cap S_{\ell+1}$, we have that $|I'|=15$. 
This contradicts the assumption that $|I'| = 16$. 
Thus all vertices $N(v) \cap R$ are assigned distinct colors.
\qed
\end{proof}

We now proceed to the correctness part. 
\begin{itemize}
    \item 
\textbf{Every vertex $v\in I$ has a uniquely colored neighbor.} 

Let $v\in S_{\ell+1} \cap I$. 
%be an isolated vertex in stripe $S_{i-1}$ 
%and $r_v$ be its representative vertex in $S_i$. 
%The vertex $r_v$ is the uniquely colored neighbor for $v$. 
By the above claim, no two vertices in $N(v) \cap R$ are assigned
the same color in phase 2.
Moreover, since $v$ is not isolated in $G$, we have $|N(v) \cap R|\geq 1$ such that it has a uniquely colored neighbor.


%\noindent
\item \textbf{The coloring in phase 2 does not upset the uniquely colored neighbors of vertices in $V\setminus I$.} 

Let $v\in V\setminus I$ and $u$ be its uniquely colored neighbor after the phase 1 coloring. 
For $v$ to not have a uniquely colored neighbor after phase 2 coloring, 
there exists a vertex $w\in N(v)$ such that $C(u)=C(w)$. 
This implies that both $u$ and $w$ are representative vertices for some vertices in 
$I$ and they are re-colored in phase 2.
This contradicts the above claim.
%By the above claim, it can not happen that $C(u)=C(w)$ where $C(u)\in \{c_1,\cdots, c_{21}\}$. 
\end{itemize}
\qed



\begin{figure}[t!]
\centering
\begin{tikzpicture}[every node/.style={node distance=1.8cm,scale=0.9}, scale = 0.5]

\tikzstyle{vertex}=[dot, draw, minimum size=8pt]
\draw[gray] (-6,2.4) -- (7,2.4);
\draw[gray] (-6,0.4) -- (7,0.4);


\draw[thick, thin] (4,3) circle (1cm);
%draw[thick, thin] (4,2) circle (6,4); 
\draw[thick, thin] (4,-0.8)  circle (1cm);
%\draw[thick, thin] (1.5,-0.8)  circle (1cm);
%\draw[thick, thin] (-0.7,-0.8)  circle (1cm); 
\draw[thick, thin] (-2.2,-0.8)  circle (1cm);
\draw[thick, thin] (-2.2,3)  circle (1cm);
\draw[black, double=black] (2.5,1.2)  circle (1cm); 
\draw[black, double=black] (-0.5,1.2)  circle (1cm); 
\draw[black, double=black] (1,2.6)  circle (1cm);
%\draw[orange, thick, dotted] (-1,-4) -- (-1,6);
%\draw[orange, thick, dotted] (3,-4) -- (3,6); 

\node at (1.2,2.6) {$v$};
%\node[above, blue]  at (5,4) {$u_2$};
\node at (2.5,1.2) {$w$};
\node  at (-0.5,1.2) {$u$}; 
\node at (-2.2, 3) {$u'''$};
\node at (4,3) {$w'''$};

\node at (-2.2,-0.8) {$u*$};
\node at (4,-0.8) {$w*$};
\node at (-6,4) {$S_{\ell+1}$};
\node at (-6,-1) {$S_{\ell-1}$}; 
\node at (-6.2, 1.4) {$S_\ell$}; 

%\node[above, blue] at (-3, 4) {$u_1$}; 
%\node[below, blue] at (-3, -2) {$u_3$}; 
%\node[below, blue] at (-0.6, -2) {$u_4$};
%\node[below, blue] at (1.4, -2) {$u_5$};
%\node[below, blue] at (3.6, -2) {$u_6$};


%\node[draw, red]  at (-1,-7.5) {u};

%\node[draw, red]  at (-10,-8) {Colors $\{4,5,6\}$};
%\node[draw, black]  at (-10,-4) {Colors $\{7,8,9\}$};
%\node[draw, blue]  at (-10,0) {Colors $\{1,2,3\}$};
%\node[draw, black]  at (-10,4) {Colors $\{4,5,6\}$};
%\node[draw, black]  at (-10,8) {Colors $\{7,8,9\}$};



\end{tikzpicture}
\caption{The vertex $v\in S_\ell +1$ is adjacent to two vertices $u$ and $w$ in $S_\ell$,  which are representative vertices for some isolated vertices. The vertices $u''', w'''\in S_{\ell +1}$ and  $u^*, w^*\in S_{\ell -1}$ belong to the set $I'$ such that in the worst case (i)  $|u_x-w_x|<4$, (ii) $|u'''_x - v_x |<3$, $|w'''_x - v_x|<3$, (iii) $|u_x - u^{*}_{x}|<2$, $|w^{*}_{x}-w_x|<2$ and 
(iv) $|u^{*}_{x}-w^{*}_{x}|<8$. 
Including $u^*$ and $w^*$, there could be at most eight isolated vertices in $I'\cap S_{\ell-1}$ between $u^*_x$ and $w^*_x$. 
%The picture describes the positions of the isolated vertices whose representative vertex $r$ is such that $u_x\leq r_x\leq w_x$. 
}
\label{fig:unitdisk}
\end{figure}

\textbf{ALTERNATIVE PROOF}








\subsection{Sriram}

We will use the following lemma.

\begin{lemma}[Theorem 5 of \cite{Sandor2017}]
\label{lem:disk_sqrt3}
Unit disk intersection graphs of height~$\sqrt{3}$ are \cfcnp{} 2-colorable.
Further, the horizontal distance between two colored vertices is greater than 1.
\end{lemma}

Note that the above lemma pertains to CFCN$^*$ coloring and not CFON$^*$ coloring. The second sentence in the above lemma is not stated in the statement of Theorem 5 in \cite{Sandor2017}, but rather in its proof. We will use the CFCN$^*$ coloring used in the above stated lemma in the process of arriving at a CFON$^*$ bound for unit disk intersection graphs. Below we reproduce the coloring process
used in the proof of the above lemma in \cite{Sandor2017}.


\begin{proof}[Coloring process used in Lemma \ref{lem:disk_sqrt3}]
Let $G=(V,E)$ be a unit disk intersection graph such that
the centers of all the disks in $G$ lie in a band of height $\sqrt{3}$. 
The vertices $V(G)$ are processed according to their non-decreasing $X$-coordinate. 
At each step of the algorithm, we choose a vertex $v$ that covers all uncolored vertices to its left, and assign the color 1 (or 2) if the previous colored vertex was assigned the color 2 (or 1). A vertex $v$ is \emph{covered} if and only if either it is colored or has a neighbor  assigned 
a color from $\{1, 2\}$. At the end, each uncolored vertex is assigned the color 0. 
It follows from the algorithm that the horizontal distance between any two colored vertices is greater than 1. 
The reader is directed to \cite{Sandor2017} for the correctness of the algorithm. 
\qed
\end{proof}

The coloring algorithm of Theorem \ref{thm:unitdisk} involves two phases. 
%We assign colors 
%$C(v)$, 
%for all the unit disks $v$ of $G$ in two phases.
In phase 1, we use 6 non-zero colors 
$C: V \to \{0\} \cup \{c_{i,0}, c_{i,1} \mid  i \in \{0,1,2\}\}$. 
WLOG we assume that the centers of all the disks have positive $Y$-coordinates.
We partition the plane into horizontal stripes $S_{\ell}$ for $\ell \in \mathbb{N}$
where each stripe is of height $\sqrt{3}$. 
We assign vertex $v$ with $Y$-coordinate $v_y$ to $S_{\ell}$ if $\sqrt{3}(\ell-1) < v_y \leq \sqrt{3}\ell$, where $G[S_\ell]$ is the graph induced on the vertices in $S_\ell$. 
Then $G[S_\ell]$ has height $\sqrt{3}$.
Using Lemma \ref{lem:disk_sqrt3}, we \cfcnp{} color vertices in $S_{\ell}$ accordingly, 
using colors $c_{i,0}, c_{i,1}$ where $i = \ell \bmod 3$. 
Let $I$ be the set of all colored vertices (assigned a non-zero color) that does not have a uniquely colored neighbor (in the CFON$^*$ sense), after phase 1.
%We will show later on that any vertex not in $I$ has a uniquely colored neighbor in $G$.

In phase 2, we will reassign colors to some vertices of $G$ to ensure a uniquely colored neighbor (in the CFON$^*$ sense) for each vertex in $I$.
For each vertex $v\in I$, choose an arbitrary \textit{representative vertex} $r(v)\in N(v)$. 
Note that the representative vertices need not be in $I$.
Also, two vertices in $I$ may share the same representative vertex.
% Let $I_1$ and $I_2$ be the vertices in $I$ that are colored $c_{i,0}$ and $c_{i,1}$, respectively, for $i \in \{0, 1, 2, 3\}$.
Let $R = \{r(v) \mid v \in I\}$ be the sets of representative vertices.
We reassign the colors of these representative vertices in the following: $C': R \to \{c'_{i,j} \mid  i \in \{0,1,2,3\}, j \in \{0,1, \ldots, 7\} \}$.
Consider a stripe $S_{\ell}$ for $\ell \in \mathbb{N}$.
We order the vertices $S_{\ell} \cap R$ non-decreasingly by their $X$-coordinate.
We consider the vertices sequentially in that order. 
If the vertex  has not been colored in phase 2 yet, then we assign it with a color from $\{c'_{i,0},\dots,c'_{i,7} \mid i \equiv \ell \bmod 4 \}$ in a cyclic manner (i.e., the vertices to be colored are assigned colors in the following sequence $c'_{i,0}, c'_{i,1}, \dots, c'_{i,7}, c'_{i,0}, \dots$). \textcolor{red}{there are two colorings. need a joint one ?}%
%The final coloring obtained is $C'$


\noindent
\textbf{Total number of colors used:} The number of colors used in phase 1 and phase 2 are 6 and 32 respectively, giving a total of 38. 

\noindent
\textbf{Correctness:} 
We now prove that the assigned coloring is a valid \cfonp{} coloring, by showing that every vertex has a uniquely colored neighbor.

First, we consider a vertex~$v\notin I$ and $v\in S_\ell$, for some $\ell$.
From the definition of ~$I$, 
$v$ is adjacent to a vertex~$u$, with $u \neq v$, colored by $C$, at the end of phase 1.
Suppose $u$ is not recolored in phase 2. 
%That is,  $u\notin R$, and since~$C$ \textcolor{red}{is a \cfcnp{} coloring of $G[S_{\ell}]$}, 
%$v$ is adjacent to a uniquely colored neighbor~$u \neq v$ in $G[S_\ell]$.
%From the coloring, 
%the distance between $v$ and other vertices in another stripe with the same color as $C(u)$ is at least $2\sqrt{3} > 2$.
In this case $u$ remains the uniquely colored neighbor of~$v$ in~$G$.

Suppose $u$ is recolored in phase 2 to some color $c'_{i,j}$.
For the sake of contradiction, let~$v$ be also adjacent to another vertex~$w$ assigned the same color~$c'_{i,j}$.
Recall that $u$ and $w$ are the representative vertices of two vertices in $I$. 
We first consider the case when $u$ and $w$ belong to different stripes. Since $u$ and $w$ are assigned $c'_{i,j}$, if they are in
different stripes, it must be the case that $|u_y-w_y|>3\sqrt{3}>5$.
But since $u, w \in N(v)$, we have that $u$ and $w$ are at a distance (as measured in the plane)
of at most 4, and hence $|u_y-w_y|\leq 4$, which is a contradiction.
Thus $u$ and $w$ cannot be in different stripes. 

Suppose that $u$ and $w$ are in the same stripe, say $S_{\ell-1}$. 
Let $u$ be the representative of a vertex $a \in I$ and $v$ be the 
representative of a vertex $b \in I$. 


that are in stripes $S_{\ell'}$ and $S_{\ell''}$, respectively, such that $i\equiv \ell' \bmod 5 \equiv \ell'' \bmod 5$. 
Note that, for any $\ell$,  no vertex in $S_\ell$ is adjacent to any vertex in $S_{\ell+3}$ or $S_{\ell-3}$. 
If $u$ and $w$ were in different stripes, then $u\in S_{\ell-3}$ and $w\in S_{\ell+3}$ or vice-versa. 


Since $(a,u,v,w,b)$ forms a path in $G$, and since two adjacent vertices in $G$ have distance at most 2, we conclude that $a$ and $b$ are at the distance of at most 8.
If $\ell \neq \ell'$, then $|\ell - \ell'| \geq 6$.
This implies $|a_y - b_y| \geq 5\sqrt{3} > 8$, a contradiction.
Hence, $a$ and $b$ are in the same stripe.
It also follows that $u$ and $w$ cannot be in two different stripes
Because $u$ and $w$ have the same color, there must be 7 other vertices in $I$ between $a$ and $b$ in terms of the $X$-coordinate.
By Lemma~\ref{lem:disk_sqrt3}, this implies $|a_x - b_x| > 8$, another contradiction.
Hence, $v$ cannot be adjacent to two vertices of the same color.

Lastly, we consider a vertex~$v$ in $I$.
Then the representative~$u$ of~$v$ is colored by $C'$.
With the same argument as above, we can conclude that~$v$ is not adjacent to another vertex with the same color.

